On Monadic Vector-Valued Integration

In recent times, there has been a growing interest in a structuralist understanding of probability, measure and integration theory. The present thesis contributes to this programme in three ways. First, we construct a commutative probability monad on the cartesian closed category of hk-spaces (also known as CGWH spaces, or weak Hausdorff k-spaces in the literature). Secondly, in order to achieve this in a seamless way, we develop the theory of paired linear hk-spaces, a functional-analytic category tailored to the duality between measures and functionals. Finally, vector-valued integration emerges naturally from the free-forgetful adjunction between paired linear hk-spaces and hk-spaces, inducing a commutative monad of compactly supported measures and leading to a theory of monadic vector-valued integration.

==> Chapters/7_Cut_Material.tex <==
\section{Lemma on $\mathcal{M}(X)$ being colimit}

\begin{lem}\label{MX_colimit}
    Let $X$ be an $hk$-space. Then $\mathcal{M}(X)$ is the sequential colimit (in $\spaces$),
        $$ \mathcal{M}(X) \:\cong\; \colim_{n\in \mathbb{N}} \{\mu \in \mathcal{M}(X) \mid \|\mu\| \leq n \}, $$
    over the inclusions of integer-radius balls centred at the origin, where $\|\cdot \|$ denotes the operator norm (with respect to the supremum norm on $C_b(X)$). 
\end{lem}
\begin{proof}
    The space $\mathcal{M}(X)$ is the union over the closed subspaces,
        $$ \mathcal{M}(X) = \bigcup_{n\in\mathbb{N}} \, \{\mu \in \mathcal{M}(X) \mid \|\mu\| \leq n \}. $$
    Therefore, it suffices to show that every compact subset of $\mathcal{M}(X)$ is contained in one of these closed subspaces (see \cref{seq_colims_in_spaces}), which is to say that every compact subset $K$ of $\mathcal{M}(X)$ is bounded in the operator norm on the Banach dual space of $C_b(X)$. To see this, notice that for every $f\in C_b(X)$, by the continuity of evaluating $\mu$ at $f$,
        $$ \sup_{\mu \in K} |\mu(f)| < \infty $$
    and apply the uniform boundedness principle. 
\end{proof}

==> Chapters/Notes.tex <==
\chapter*{Notes and Planning}

\section{Prioritised TODO list}

\begin{displaycomment}
    Prioritised TODOs:
    \begin{itemize}
        \item check terminology: $k$-Hausdorff spaces vs hk-space; the ``L-dual'' vs just ``dual'' or ``dual taken in...''; morphism of paired linear hk-space vs linear operator; compactum vs compact Hausdorff space; ...
        \item Cosmetic TODOs: change font size; change hom to Hom; polish references; ...
        \item bibliography not as appendix!
        \item capitalisation of section titles
    \end{itemize}
\end{displaycomment}





\section{Tables for appendix}


\cref{defn_paired_lin_hk_sp}

\cite[Proposition 1.7]{scholze2019condensed}
\cite[Lemma 4.14]{sclausen2020lectures}
\cite[p. 15]{clausen2022condensed}
\cite{lucien1971compactological}
\cite[p. 370]{akbarov2022stereotype}
\cref{sepobjs_corefl_subcat_of_little_chu}
\cite[p. 71]{schaefer1971topological}
\cite{prosmans2000homological}
\cite[1.3]{porta1972compactly}

\cite[Corollary 3.8]{blute2010convenient}
\cite[Lemma 3.18]{blute2010convenient}
\cite[Lemma 2.6.5]{frolicher1988linear}

\cite{kriegl1997convenient}
\cref{defn_k_ification}
\cref{defn_kloc}

% adjunctions table
% ----------------------------------------------------------
\begin{table}[]
\begin{tabular}{ccl}
Adjunction between...                                     & ...and...                                          & Reference                                                                                                                                                                                                                                                                            \\
$\mathsf{L}$                                              & $r\mathsf{Vect}(hk\mathsf{Top})$                   & \textbackslash{}cref\{sepobjs\_corefl\_subcat\_of\_little\_chu\}                                                                                                                                                                                                                     \\
$\mathsf{Vect}(hk\mathsf{Top})$                           & $\mathsf{Cond}(\mathsf{Vect})_{q.s.}$              & \textbackslash{}cite{[}Proposition 1.7{]}\{scholze2019condensed\}                                                                                                                                                                                                                    \\
$hk\mathsf{Top}$                                          & $\mathsf{Cond}(\mathsf{Set})_{q.s.}$               & \textbackslash{}cite{[}Proposition 1.7{]}\{scholze2019condensed\}                                                                                                                                                                                                                    \\
$\mathsf{Cond}(\mathsf{Set})_{q.s.}$                      & $\mathsf{Cond}(\mathsf{Set})$                      & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cite{[}Lemma 4.14{]}\{sclausen2020lectures\},\\ see \textbackslash{}cite{[}p. 15{]}\{clausen2022condensed\} \\ for the equivalence to the ``compactological \\ spaces'' of \textbackslash{}cite\{lucien1971compactological\}\end{tabular} \\
\multicolumn{1}{l}{$\mathsf{Cond}(\mathsf{Vect})_{q.s.}$} & \multicolumn{1}{l}{$\mathsf{Cond}(\mathsf{Vect})$} & \textbackslash{}cite{[}Lemma 4.14{]}\{sclausen2020lectures\}                                                                                                                                                                                                                         \\
$\mathsf{Vect}(hk\mathsf{Top})$                           & $lk\mathsf{LCTVS}$                                 & \textbackslash{}cref\{kloc\_conv\_equiv\_ksat\_lctvs\}                                                                                                                                                                                                                               \\
$\mathsf{LCTVS}_{k\mathrm{c}}$                            & $\mathsf{LCTVS}$                                   & \textbackslash{}cite{[}Theorem 3.3.1{]}\{akbarov2022stereotype\}                                                                                                                                                                                                                     \\
$\mathsf{Ste}$                                            & $\mathsf{LCTVS}_{k\mathrm{c}}$                     & \textbackslash{}cite{[}Theorem 3.3.15, Theorem 4.1.1{]}\{akbarov2022stereotype\}                                                                                                                                                                                                     \\
$\mathsf{Vect(Born)}$                                     & $\mathsf{Born}$                                    & \begin{tabular}[c]{@{}l@{}}with the basic constructions \\ given in \textbackslash{}cite\{prosmans2000homological\},\\ free objects can be constructed \\ as in the proof of \textbackslash{}cref\{free\_lin\_hk\_sp\_existence\}\end{tabular}                                      
\end{tabular}
\end{table}






% categories table
% -----------------------------------------
% -----------------------------------------------------------

\begin{table}[]
\begin{tabular}{llllll}
\cline{1-4}
Category                              & Objects                                                                                                     & References                                                                                                                                                 & Category                         & Objects                                                                                                                 & References                                                                                                                                               \\ \hline
$hk\mathsf{Top}$                      & \begin{tabular}[c]{@{}l@{}}$hk$-spaces/\\ CGWH spaces\end{tabular}                                          & \textbackslash{}cref\{defn\_k\_sp\_hk\_sp\}                                                                                                                & $\mathsf{LCTVS}$                 & \begin{tabular}[c]{@{}l@{}}Hausdorff locally convex\\ topological vector spaces\end{tabular}                            & ---                                                                                                                                                      \\
$\mathsf{Vect}(hk\mathsf{Top})$       & linear $hk$-spaces                                                                                          & \textbackslash{}cref\{def\_lin\_hk\_space\}                                                                                                                & $lk\mathsf{LCTVS}$               & \begin{tabular}[c]{@{}l@{}}compactly determined\\ LCTVS\end{tabular}                                                    & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cref\{defn\_ksat\_l\}\\ \textbackslash{}cite\{porta1972compactly\}\end{tabular}                               \\
$r\mathsf{Vect}(hk\mathsf{Top})$      & \begin{tabular}[c]{@{}l@{}}replete linear \\ $hk$-spaces\end{tabular}                                       & \textbackslash{}cref\{ex\_repl\_lin\_sk\_sp\}                                                                                                              & $\mathsf{LCTVS}_{k\mathrm{c}}$   & \begin{tabular}[c]{@{}l@{}}$k$-complete/\\ pseudocomplete LCTVS\end{tabular}                                            & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cref\{defn\_kcompl\_seqcompl\}\\ \textbackslash{}cite{[}p. 370{]}\{akbarov2022stereotype\}\end{tabular}       \\
$\plin$                               & \begin{tabular}[c]{@{}l@{}}paired linear \\ $hk$-spaces\end{tabular}                                        & \textbackslash{}cref\{defn\_paired\_lin\_hk\_sp\}                                                                                                          & $lk\mathsf{LCTVS}_{k\mathrm{c}}$ & \begin{tabular}[c]{@{}l@{}}compactly determined\\ $k$-complete LCTVS\end{tabular}                                       & (see above)                                                                                                                                              \\
$\mathsf{Cond(Set)}$                  & condensed sets                                                                                              & \textbackslash{}cite\{scholze2019condensed\}                                                                                                               & $b\mathsf{LCTVS}$                & bornological LCTVS                                                                                                      & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cite{[}p.$\sim$71{]}\{schaefer1971topological\}\\ \textbackslash{}cite\{blute2010convenient\}\end{tabular}    \\
$\mathsf{Cond}_{q.s.}(\mathsf{Set})$  & \begin{tabular}[c]{@{}l@{}}quasi-separated (q.s.) \\ condensed sets/\\ compactological spaces\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cite{[}p.$\sim$15{]}\{clausen2022condensed\}, \\ \textbackslash{}cite\{lucien1971compactological\}\end{tabular} & $st\mathsf{CBS}$                 & \begin{tabular}[c]{@{}l@{}}separated, topological \\ convex bornological \\ vector spaces (CBS)\end{tabular}            & \textbackslash{}cite{[}p.$\sim$10{]}\{blute2010convenient\}                                                                                              \\
$\mathsf{Cond(Vect)}$                 & \begin{tabular}[c]{@{}l@{}}condensed vector \\ spaces\end{tabular}                                          & \textbackslash{}cite\{scholze2019condensed\}                                                                                                               & $\mathsf{Conv}$                  & \begin{tabular}[c]{@{}l@{}}``convenient vector spaces''\\ (Mackey-complete, \\ separated, topological CBS)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cite\{kriegl1997convenient\} \\ \textbackslash{}cite{[}Definition 3.15{]}\{blute2010convenient\}\end{tabular} \\
$\mathsf{Cond}_{q.s.}(\mathsf{Vect})$ & \begin{tabular}[c]{@{}l@{}}quasi-separated (q.s.)\\ condensed/compactological \\ vector spaces\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbackslash{}cite{[}p.$\sim$15{]}\{clausen2022condensed\}, \\ \textbackslash{}cite\{lucien1971compactological\}\end{tabular} & $\mathsf{Ste}$                   & stereotype spaces                                                                                                       & \textbackslash{}cite{[}p.$\sim$477{]}\{akbarov2022stereotype\}                                                                                           \\ \hline
\end{tabular}
\end{table}




























































\section{Notes on Introduction}


\subsection{A comparison of ``convenient'' functional analytic categories}\label{sec_some_proposed_convenient_settings}

TODO : rewrite section; make ``big picture'' \par 

We now review some known examples of closed monoidal categories of complete-topological-vector-space-like objects and how they relate to (replete) linear $hk$-spaces.

\begin{enumerate}[1.]
    \item \emph{Full subcategories of $\lctvs$:} These include \emph{Mackey-complete, bornological} locally convex spaces (called ``convenient vector spaces'' by Kriegl and Michor, who use them as a basis for infinite-dimensional calculus and differential geometry, see \cite[Theorem 2.14]{kriegl1997convenient}, and \cite[Theorem 4.2]{blute2010convenient}), \emph{quasi-complete, barrelled} locally convex spaces (see \cite[(10.6) Theorem]{ligon1978galois}), \emph{pseudo-complete, pseudo-saturated} locally convex spaces (called ``stereotype spaces'', which are even \emph{$*$-autonomous}, see \cite[Theorem 4.4.31]{akbarov2022stereotype}). An approach which is quite similar to the setting of replete linear $hk$-spaces is that of Seip \cite{seip1979convenient} (see also \cite{frolicher1972dualitatstheorie}), who, like Kriegl and Michor, developed this setting for the purposes of infinite dimensional calculus. His category is based on $k$-spaces and equivalent to (although this is perhaps a less natural point of view) the category of \emph{sequentially complete, compactly determined} locally convex spaces (see \cref{defn_kcompl_seqcompl}), Chapter 5, where we will lay out the precise relation of this category to our setting).  All of the aforementioned categories come with a closed symmetric monoidal structure.
    \item \emph{Convergence spaces, compactological spaces and condensed mathematics:} Instead of passing to a cartesian closed subcategory of topological spaces as a ``base category'', several cartesian closed enlargements of $\topsp$ have been considered, including \emph{convergence spaces} \cite{beattie2013convergence}, \emph{compactological spaces} \cite{lucien2006compactological}, and most recently, \emph{condensed sets} \cite{scholze2019condensed} (which can be seen as a generalisation of compactological spaces, see \cite[Proposition 1.2]{sclausen2020lectures}). The condensed approach essentially entails the compactological one and is most closely related to ours in that the category of $hk$-spaces embeds into that of condensed sets. In addition, we have seen that the replete linear $hk$-spaces can be viewed as certain \emph{$\mathcal{M}$-complete condensed vector spaces}.  %(( TODO : make separate point for condensed maths and emphasise that linear $hk$-spaces are a special case condensed vector spaces. )) 
    % TODO : replete spaces embed into 
\end{enumerate}



\section{Good open problems}

\begin{itemize}
    \item Are paired linear $k$-spaces a (co-)differential category?
    \item Analogous development possible internal to a category of smooth spaces? E.g. are paired linear diffeological a (co-)differential category?
    \item codensity monad: further justification that setting is ``right''.
\end{itemize}

Some more possible applications:

\begin{enumerate}
    \item characterise compact subsets of $\mathcal{M}(X)$ via Arzela-Ascoli.
    \item Every paired linear QCB space is a (topological linear) quotient of $\mathcal{M}_c(X)$ for $X$ a separable metric space. Is this useful?
    \item \cite{hager1969approximation} is a sequential Stone-Weierstrass theorem for lindelöf (hence QCB) spaces. It implies that a point-separating $*$-sub-algebra of $C(X)$ for $X$ QCB, completely regular and Hausdorff is dense (in the natural topology). The question is now: is complete regularity really used or just assumed out of laziness? I think the answer is that it's not necessary, as one can pass to the completely regular reflection and apply Hager's result there.
    \item Does Corollary 7.3.4 imply that every Baire measure on a Brauner space is a Radon measure?
\end{enumerate}

\section{Some possible additions to the section on QCB spaces}

\begin{prop}\label{compactness_in_QCB_spaces}
    Let $X$ be a QCB space and $K\subseteq X$ be a subset. Then the following are equivalent:
    \begin{enumerate}[1.]
        \item $K$ is compact.
        \item $K$ is sequentially compact (which means that every sequence in $K$ has a convergent subsequence).
        \item $K$ is countably compact (meaning that every \emph{countable} cover has a finite subcover).
    \end{enumerate}
    Moreover, any compact sequentially Hausdorff QCB space is metrisable and any compact subset of a QCB space is a QCB space.
\end{prop}
\begin{proof}
     The one between compactness and countable compactness holds in any sequential space \cite[Theorem 3.10.31]{engelking1989general}, so we only need to show the equivalence between sequential compactness and countable compactness. (( TODO : complete proof ))
\end{proof}

\begin{remark}
    The equivalences in Proposition \ref{compactness_in_QCB_spaces} are asserted without proof in \cite[Proposition 4.8]{battenfeld2007convenient}.
\end{remark}

\subsubsection{Separable hemicompact $k$-spaces are QCB spaces} (( TODO : do I reall yned this? :: An observation which we will need later on is that every separable hemi.. ))

\subsubsection{Sequentially Hausdorff QCB spaces are $k$-Hausdorff} (( TODO : do I really need this ? )) 





\section{Some notes on CGWH vs condensed}

Having thought about this again, I think it follows from generalities. Specifically:

\begin{lem}
    Let $S$ be a site with finite products and let $\underline{\cdot}:\mathsf{C}\hookrightarrow \mathsf{Sh}(S)$ be a reflective subcategory. Suppose that we have a fully faithful, product-preserving functor $\iota: S\hookrightarrow \mathsf{C}$ such that 
    $\underline{\cdot} \circ \iota: S \to \mathsf{Sh}(S)$ is the Yoneda embedding $y$.
    Then $\mathsf{C}$ is an exponential ideal in $\mathsf{Sh}(S)$. 
\end{lem}
\begin{proof}
    Let $Y\in \mathsf{C}$ and $K\in S$. Then for all $L\in S$:
    \begin{align*}
        \underline{Y}^{y(K)}(L) &\cong \hom(y(L), \underline{Y}^{y(K)}) \\
        &\cong \hom(y(L) \times y(K), \underline{Y})\\
        &\cong \hom(y (L \times K), \underline{Y}) \\
        &\cong \hom( \underline{\iota(L \times K)}, \underline{Y}) \\
        &\cong \hom(\iota(L\times K), Y) \\
        &\cong \hom(\iota(L)\times \iota(K), Y) \\
        &\cong \hom(L, Y^{\iota(K)}) \\
        &\cong \hom(\underline{L}, \underline{Y^{\iota(K)}})\\
        &\cong \underline{Y^{\iota(K)}}(L).
    \end{align*}
    Hence, 
        $$ \underline{Y}^{y(K)} \cong \underline{Y^{\iota(K)}}$$
    Now, every $X\in \mathsf{Sh}(S)$ is the colimit of representables, written with an abuse of notation as follows,
        $$ X \cong \colim_{K\to X} y(K). $$
    Therefore, if $Y\in \mathsf{C}$ and $X\in \mathsf{Sh}(S)$, then 
    \begin{align*}
        \underline{Y}^X &\cong \lim_{K\to X} \underline{Y}^{y(K)}\\ 
        &\cong \lim_{K\to X} \underline{Y^{\iota(K)}} \\
        &\cong \underline{\lim_{K\to X} Y^{\iota(K)}} \\
        &\cong \underline{Y^{\colim_{K\to X} \iota(K)}} \\ 
        &\cong \underline{Y^{X(*)_{\mathrm{top}}}}.
    \end{align*}
\end{proof}

$$ \underline{Y}^X \cong \lim_K \underline{Y}^\underline{K} \cong \lim_K \underline{Y^K} \cong \underline{\lim_K Y^K} \cong \underline{Y^K} $$

Reflective subcategory of sheaf category inherits exponentials:

$$ \underline{Y}^\underline{K}(L) \cong \hom(\underline{L}, \underline{Y}^\underline{K}) \cong \hom(\underline{L} \times \underline{K}, \underline{Y}) \cong \hom(\underline{L \times K}, \underline{Y}) \cong \hom(L\times K, Y) \cong \hom(L, Y^K) \cong \hom(\underline{L}, \underline{Y^K})\cong \underline{Y^K}(L)$$

\section{Smith Duality for QCB spaces}

\begin{defn}
    ((TODO : replete linear $k$-/QCB space ))
\end{defn}

\begin{lem}
    Let $V$ be a replete linear $k$-space and let $K\subseteq V$ be compact. Then the closed convex hull,
        $$ C := \overline{\mathrm{conv}(K)}, $$
    of $K$ is also compact.
\end{lem}
\begin{proof}
    Since $V$ is replete, the evaluation map, 
    $$e: V \to C(V^{\wedge}), \;\; x \mapsto (f \mapsto f(x))$$
    is a closed embedding, so $C$ is compact if, and only if, the image, 
        $$ C' := \eta(C) = \overline{\mathrm{conv}(\eta(K))} \subseteq C(V^{\wedge}),$$
    is compact. Let 
        $$ C'' := \overline{\mathrm{conv}(\eta(K))}^{c.o.} \subseteq \cco(V) $$
    be the closed convex hull of $\eta(K)$, \emph{with the closure taken in the compact-open topology}. The space $\cco(V)$ of continuous functions on $V$ with the compact-open topology is a Hausdorff locally convex topological vector space (short: LCTVS) which is furthermore complete, because $V$ is a $k$-space. Therefore, $C''$ is compact in $\cco(V)$ (as the closed convex hull of a compact set in a complete LCTVS always is, see TODO). The compact subsets of $\cco(V^\wedge)$ and $C(V^\wedge)$ agree, implying that $C''$ is compact in $C(V^\wedge)$, too. Moreover, $C' \subseteq C''$, since the topology of $C(V^\wedge)$ is finer than that of $\cco(V^\wedge)$. Hence, as a closed subset of a compact set, $C$ is compact, which is what we wanted to show.
\end{proof}

\begin{lem}
    Let $V$ be a linear QCB space. Then every continuous linear functional on $V^\wedge$ is also continuous with respect to the compact-open topology on $V^\wedge$.
\end{lem}
\begin{proof}
    Let $\phi\in V^{\wedge\wedge}$ be a continuous linear functional on $V^\wedge$. Denote by 
        $$ V^{*^{c.o.}} \subseteq \cco(V) $$
    the dual of $V$ endowed with the compact-open topology, i.e.~the (ordinary) subspace topology induced from $\cco(V)$. We want to show that $\phi$ is continuous on $V^{*^{c.o.}}$. Since $V$ is a QCB space, so is $V^\wedge$ (see Proposition TODO). As a QCB space, $V^\wedge$ is separable and therefore, with its coarser topology, $V^{*^{c.o.}}$ is separable, too. Let $D\subseteq V^{*^{c.o.}}$ be a countable dense subspace of $V^{*^{c.o.}}$. The functional $\phi$ is sequentially continuous on $V^{*^{c.o.}}$ (this is what continuity of $\phi$ on $V^\wedge$ amounts to) and in particular, sequentially continuous on $D$. But as $D$ is countable, this already implies that $\phi$ is continuous on $D$ (with respect to the subspace topology induced from $V^{*^{c.o.}}$). Now, since $D\subseteq V^{*^{c.o.}}$ is dense, there exists a unique extension of $\phi$ from $D$ to a continuous linear functional on $V^{*^{c.o.}}$, and this extension is necessarily $\phi$ itself. Hence, $\phi$ is continuous on $V^{*^{c.o.}}$, which is what we wanted to show. 
\end{proof}



\begin{thm}
    Let $V$ be a linear QCB space. Then the canonical evaluation map 
        $$\eta: V \to V^{\wedge\wedge}, \;\;\; x\mapsto \langle x,  - \rangle $$
    is surjective.  
\end{thm}
\begin{proof}
    (( TODO : Q: can I do this without passing to locally convex spaces?? )) Let $E$ be a complete locally convex Hausdorff topological vector space such that $V=kE$. Then a linear functional is continuous on $V$ is, and only if, it is continuous on $E$ (TODO : is it?). In other words, the underlying sets of $V^\wedge$ and $E^{*^{c.o.}}$ agree: 
        $$ |V^\wedge| = |E^{*^{c.o.}}|. $$
\end{proof}

\begin{cor}
    (( duality thm )) 
\end{cor}

\section{Old section on false proof of duality theorem}

\subsection{Duality of linear QCB spaces}

The goal of this section is to extend the (separable case of) the Smith duality theorem to the case of \emph{replete} linear QCB spaces. Let us first state the relevant definition.

\begin{defn}
    A linear $k$-space is \emph{replete} if the canonical map $\eta: V \to V^{\wedge\wedge}$ is a closed embedding. 
\end{defn}

As a consequence of Smith duality, every Fréchet space and every Brauner space is replete and consequently, every separable Fréchet space is a replete linear QCB space. Moreover, it will follow from developments of the general theory of duality in closed symmetric monoidal categories (see \cref{sec_triple_dualisation_lem_and_sep_obj}), that replete linear QCB spaces are closed under the formation of spaces of continuous linear maps, admit a natural notion of tensor product and have all countable limits and colimits. Therefore, they contain many, if not most spaces that arise in applications. Moreover, in contrast to the duality between Fréchet and Brauner spaces, the duality provided here will be of a symmetric kind, endowing the category of replete linear QCB spaces with the structure of a \emph{$*$-autonomous category} (see \cref{sec_star_aut_cats}). \par 
The proof of the duality theorem for replete linear QCB spaces (\cref{thm_duality_replete_lin_QCB_spaces}) will require two lemmas and several different notions of dual space. For the sake of clarity, let us introduce the following notations.

\begin{notation}
    Let $V$ be a vector space equipped with some topology (e.g.~$V$ may be a linear $k$-space or a topological vector space).
    \begin{enumerate}[1.]
        \item Write $V'$ for the set of all continuous linear functionals on $V$, not endowed with any topology.
        \item Write $V^{*[w]}$ for the LCTVS resulting from endowing $V'$ with the topology of pointwise convergence, i.e~the topology induced by the family of seminorms
            $$ \|\phi\|_{x} := |\phi(x)|. \qquad (x\in V)$$
        When $V$ is a topological vector space, this is nothing but the weak-$*$ topology.
        \item Write $V^{*[c.o.]}$ for the LCTVS resulting from endowing $V'$ with the compact-open topology, i.e.~the topology induced by the family of seminorms
            $$ \|\phi\|_K := \sup_{x\in K} |\phi(x)| \qquad (K\subseteq V \;\text{compact})$$
    \end{enumerate}
\end{notation}

Next is the key lemma.

(( WARNING/TODO : the proof of following lemma was false )) 

\begin{lem}\label{functl_cont_wrt_co_toplgy}
    Let $V$ be a linear $k$-space. Then every continuous linear functional on the natural dual $V^\wedge$ is also continuous on the compact-open dual $V^{*[c.o.]}$. In symbols, 
        $$(V^\wedge)' = (V^{*[c.o.]})'.$$
\end{lem}
\begin{proof}
    ((TODO : maybe try using Chapter 5: try prove that a closed absolutely convex neighbourhood in the LCTVS $lk V^{*[c.o.]}$ is in fact a neighbourhood in $V^{*[c.o.]}$ by writing it as the polar of a compact subset of $V$; hopefully it suffices to write it as a pre-polar of a compact subset of $V^{\wedge\wedge}$ which could work by Arzela-Ascoli )).
\end{proof}

The following lemma is essentially due to the fact that \emph{repleteness} implies a form \emph{completeness} (a precise formulation of this will be given in Chapter 5, \cref{sec_compl_of_lin_k_sp}). 

\begin{lem}\label{lem_closed_conv_hull_cpct}
    Let $V$ be a replete linear $k$-space and let $K\subseteq V$ be compact. Then the closed convex hull,
        $$ C := \overline{\mathrm{conv}(K)}, $$
    of $K$ is also compact.
\end{lem}
\begin{proof}
    Since $V$ is replete, the evaluation map, 
    $$\eta: V \to C(V^{\wedge}), \;\; x \mapsto (f \mapsto f(x))$$
    is a closed embedding, so $C$ is compact if, and only if, the image, 
        $$ C' := \eta(C) = \overline{\mathrm{conv}(\eta(K))} \subseteq C(V^{\wedge}),$$
    is compact. Let 
        $$ C'' := \overline{\mathrm{conv}(\eta(K))}^{c.o.} \subseteq \cco(V) $$
    be the closed convex hull of $\eta(K)$, \emph{with the closure taken in the compact-open topology}. The space $\cco(V)$ of continuous functions on $V$ with the compact-open topology is a Hausdorff locally convex topological vector space (short: LCTVS) which is furthermore complete, because $V$ is a $k$-space. Therefore, $C''$ is compact in $\cco(V)$ (as the closed convex hull of a compact set in a complete LCTVS always is, see \cite[p. 50, 4.3 Corollary]{schaefer1971topological}). The compact subsets of $\cco(V^\wedge)$ and $C(V^\wedge)$ agree (\cref{cpct_sets_in_kififcation}), implying that $C''$ is compact in $C(V^\wedge)$, too. Moreover, $C' \subseteq C''$, since the topology of $C(V^\wedge)$ is finer than that of $\cco(V^\wedge)$. Hence, as a closed subset of a compact set, $C$ is compact, which is what we wanted to show.
\end{proof}

We are now ready to prove:

\begin{thm}[Duality theorem for replete linear QCB spaces]\label{thm_duality_replete_lin_QCB_spaces}
    Let $V$ be a replete linear QCB space. Then the canonical map $\eta: V \to V^{\wedge\wedge}$ is an isomorphism.
\end{thm}
\begin{proof}
    Since $V$ is replete, $\eta$ is a closed embedding, by definition. Hence, it suffices to show that $\eta$ is surjective. \par 
    Let $\chi \in V^{\wedge\wedge}$. By \cref{functl_cont_wrt_co_toplgy}, $\chi$ is continuous on $V^{*[c.o.]}$, so the subset
        $$ U := \{\phi\in V^{*[c.o.]}\mid \mathrm{Re}\: \chi(\phi) < 1\} \subseteq V^{*[c.o.]}$$
    is open in $V^{*[c.o.]}$. Therefore, by the definition of the topology on $V^{*[c.o.]}$ in terms of seminorms, there exists a compact subset $K_0\subseteq V$ and $\epsilon>0$ such that 
    \begin{equation}\label{co_open_contained_in_U}
        \{\phi \in V^{*[c.o.]}\mid \sup_{x\in K_0} |\phi(x)| < \epsilon \} \subseteq U.
    \end{equation}
    Let 
        $$ K := \overline{\mathrm{conv}(\epsilon^{-1} D \cdot K_0)} \subseteq V $$
    be the closed convex hull of 
        $$\epsilon^{-1} D \cdot K_0 = \{\epsilon^{-1} \lambda x \in V \mid x\in K_0,\: \lambda\in \mathbb{K}, \: |\lambda|\leq 1\},$$ 
    where $D\subseteq \mathbb{K}$ is the unit disk in $\mathbb{K}$. We claim that $\chi \in \eta(K)$, which would complete the proof. \par 
    Suppose to the contrary that $\chi \not\in \eta(K)$. The strategy is now to apply the Hahn-Banach separation theorem to separate $\chi$ and $\eta(K)$ by a hyperplane, leading to a contradiction.
    To this end, notice first that $K$ is compact (by \cref{lem_closed_conv_hull_cpct}) and absolutely convex (by construction; \emph{absolutely} convex meaning that in addition to being convex, $K$ is also closed under multiplication by scalars $\lambda\in \mathbb{K}$ with $|\lambda|\leq 1$). Now, being the image of a compact absolutely convex set, $\eta(K)$ is a compact and absolutely convex subset of $V^{\wedge\wedge}$. We claim that $\eta(K)$ is also compact in the weak-$*$ dual $(V^{*[c.o.]})^{*[w]}$. This is because $(V^\wedge)' = (V^{*[c.o.]})'$ (by \cref{functl_cont_wrt_co_toplgy}) and the identity map
        $$(V^\wedge)^\wedge \to (V^{*[c.o.]})^{*[w]}$$
    is continuous. By the Hahn-Banach separation theorem, we can now strictly separate the compact convex subset $\eta(K)$ from the closed convex subset $\{\chi\}$ by a hyperplane in $(V^{*[c.o.]})^{*[w]}$. This means that there exists a linear functional $\psi_0 \in ((V^{*[c.o.]})^{*[w]})'$ and a $t\in \reals$ such that for all $\xi\in \eta(K)$,
        $$ \mathrm{Re}\: \psi_0(\xi) < t < \mathrm{Re}\: \psi_0(\chi). $$
    By a corollary of the Hahn-Banach theorem (see, for example, \cite[p. 67f, 3.14]{rudin1991functional}), every continuous linear functional on the weak-$*$ dual of an LCTVS is given by a point evaluation functional. Applying this to $\psi_0$, this means that there exists a $\psi \in V^{*[c.o.]}$ such that for all $\xi \in (V^{*[c.o.]})^{*[w]}$, 
        $$ \psi_0(\xi) = \xi(\psi). $$
    Hence, we have that 
        $$ \sup_{x\in K} \mathrm{Re}\: \psi(x) < t < \mathrm{Re}\: \chi(\psi). $$
    Since $K$ contains the origin, $0 < \sup_{x\in K} \mathrm{Re}\: \psi(x)$ and therefore, $0 < t$. 
    Dividing the above inequalities by $t$ and using that $K$ is \emph{absolutely} convex, we see that
    \begin{equation}\label{hahn_banach_sep_chi}
        \sup_{x\in K} |(t^{-1}\,\psi)(x)| < 1 < \mathrm{Re}\: \chi(t^{-1} \psi).
    \end{equation}
    By construction,  
    $$ \{\phi \in V^{*[c.o.]}\mid \forall x\in K: |\phi(x)| < 1 \} \;\;\subseteq\;\; \{\phi \in V^{*[c.o.]}\mid \forall x\in K_0: |\phi(x)| < \epsilon \}, $$
    and hence, by \eqref{co_open_contained_in_U}, we have that 
    \begin{equation}\label{basic_co_open_in_U}
        \{\phi \in V^{*[c.o.]}\mid \forall x\in K: |\phi(x)| < 1 \} \subseteq U.
    \end{equation}
    By \eqref{hahn_banach_sep_chi}, this implies that $t^{-1}\psi \in U$. But \eqref{hahn_banach_sep_chi} also implies that $1 < \mathrm{Re}\: \chi(t^{-1} \psi)$, so the definition of $U$ yields that $t^{-1} \psi \not\in U$, a contradiction. 
\end{proof}


% sketch for complex version: use hahn banach extension theorem (applied to compact-open topology) to exetend $\chi\in V^{\wedge\wedge}$ to a functional on $(V_\reals)^\wedge$, where $V_\real$ is $V$ viewed as a real linear QCB space. This is given by point evaluation, by the real case of the theorem. done.

% possible further TODOs for later: Hahn-Banach for replete linear QCB spaces; regular epimorphisms of replete linear QCB spaces are quotient maps --> this would be enough to imply that replete linear QCB spaces are equivalently Mc-modules!



\section{Old section on $k$-local convexification}

\subsection{The $k$-local convexification of a linear $k$-space}

\begin{defn}[$k$-Local convexification]
    Let $V$ be a linear $k$-space.
    \begin{enumerate}
        \item We define the \emph{$k$-local convexification} of $V$, which we denote by $\lconvn V$, as the image of $V$ in $\chi$ under the canonical map $\eta^V: V \to \chi$. Denote the co-restriction of $\eta^V$ to $cV$ by
        	$$ j^V : V \to \lconvn V. $$
        \item If $f:V\to W$ is a continuous linear map to another linear $k$-space $W$, we define
            $$ \lconvn f: \lconvn V \to \lconvn W $$
        as the restriction of 
            $$ f^{\wedge\wedge}: \chi \to W^{\wedge\wedge}, \;\;\; \chi \mapsto (\phi \mapsto \chi(\phi \circ f))$$
        to $\lconvn V$. In this way, we obtain the \emph{$k$-local convexification functor} 
            $$ \lconvn: \vect \to \klctvs, \;\;\; V \to \lconvn V, \;\; f\to \lconvn f. $$
    \end{enumerate}
\end{defn}

\begin{prop}[Universal property of local convexification]\label{uni_prop_lconvn}
    Let $V$ be a linear $k$-space. Then 
    \begin{enumerate}[1.]
    	\item $V$ is $k$-locally convex if, and only if,
    		$j^V: V \to \lconvn V$
    	is an isomorphism. 
        \item The natural map 
        	$$i^{\lconvn V}: \lconvn V \to \lconvn \lconvn V$$
        	is an isomorphism, i.e. the $k$-local convexification of $V$ is $k$-locally convex.
        \item If $f:V \to W$ is a continuous linear map to some $k$-locally convex linear $k$-space $W$, then there exists a unique continuous linear map $\overline{f}: \lconvn V \to W$ such that the following diagram commutes:
            \[\begin{tikzcd}
	        {\lconvn V} \\
	        V & W
	       \arrow["f"', from=2-1, to=2-2]
	       \arrow["{j^V}", from=2-1, to=1-1]
	       \arrow["{\overline{f}}", from=1-1, to=2-2]
            \end{tikzcd}\]
        Hence, the $k$-local convexification functor $\lconvn$ is left adjoint to the inclusion functor
            $$  \klctvs \hookrightarrow \vect. $$
        \item Moreover, this adjunction is ``enriched'', in that we have a natural isomorphism of linear $k$-spaces:
            $$ \overline{\,\cdot\,}: \:L(\lconvn V,W) \cong L(V, W), \;\;\; f \mapsto \overline{f}. $$
        \end{enumerate}
\end{prop}
\begin{proof}
    This is completely analogous to the proof of \ref{uni_prop_scompl}:
    \begin{enumerate}[1.]
    	\item This is clear.
        \item We have seen in proposition \ref{ksubsp_locally_convex} that a linear $k$-subspace of a $k$-locally convex linear $k$-space is again locally convex. Since 
            $$\lconvn V \subseteq \chi \subseteq C(V^\wedge)$$ 
        are inclusions of linear $k$-subspaces and $C(V^\wedge)=k\cco(V^\wedge)$ is $k$-locally convex, this implies that $\scompl V$ is $k$-locally convex, as well.
        \item Since $W$ is $k$-locally convex, $j^W$ is an isomorphism. Let $r^W$ denote its inverse and define
        	$$\overline{f}:= r^W \circ \scompl f : \scompl V \to W$$
        Then by naturality of $j$, $j^W \circ f = \scompl f \circ i^V$ and hence, 
            $$ f = r^W \circ j^W \circ f = r^W \circ \scompl f \circ j^V  = \overline{f} \circ j^V, $$
        showing that the required diagram commutes. To see that $\overline{f}$ is unique with this property, suppose that $\tilde{f} \circ j^V = f$, as well. Then $\tilde{f} \circ j^V = \overline{f} \circ j^V$ and since $j^V$ is surjective, this implies $\tilde{f} = \overline{f}$.
        \item By cartesian closure of $\spaces$, the map $f \to \overline{f}$ is continuous, with continuous inverse given by $g \mapsto g \circ j^V$. Therefore, the map $f \to \overline{f}$ (which is clearly also linear) is a homeomorphism, as claimed.
    \end{enumerate}
\end{proof}

\section{Old section of free LCTVS vs free replete linear k-spaces}

\section{\texorpdfstring{Relation between Free Replete Linear $hk$-Spaces and Free Locally Convex Spaces}{Relation between Free Replete Linear hk-Spaces and Free Locally Convex Spaces}}

In this section, we will show that the free replete linear $hk$-space $\mnd(X)$ on an $hk$-space $X$ (which also the underlying $hk$-space of the free paired linear $hk$-space) is closely related to the \emph{free locally convex topological vector space (LCTVS)} on a topological space, the construction of which we will recall below. A comprehensive treatment on free topological vector spaces is given in \cite{flood1975free}. \par
Specifically, we shall see that the faithful (``forgetful'') functor 
    $$ k: \lctvs \to \spaces $$
from the category $\lctvs$ of LCTVS to that of $k$-spaces, given by $k$-ification of the underlying topological space, has a left adjoint
    $$ M_{LC}: \spaces \to \lctvs, $$
the \emph{free LCTVS} on a $k$-space, such that:
    $$ \mnd = \scompl k M_{LC}, $$
where $\scompl$ denotes the repletion functor (see \cref{defn_repletion}).

\subsection{The free locally convex space on a topological space}
The construction of the free locally convex spaces on a \emph{topological space} is well known (see \cite[p. 6]{flood1975free}). Let us recall its details.

\begin{defn}[Free locally convex space $M_{LC}$]
    Let $X$ be a topological space. The \emph{free not-necessarily-Hausdorff locally convex topological vector space} $M_{LC}^0(X)$ on $X$ is the free (algebraic) vector space on $X$ endowed with the the family of all seminorms $\|\cdot\|$ on $M_{LC}^0(X)$ such that 
        $$ (x,y)\mapsto \|x-y\| $$
    is continuous on $X\times_{\topsp} X$ (where the difference $x-y$ is taken in $M_{LC}^0(X)$). The \emph{free LCTVS} $M_{LC}(X)$ is the Hausdorff quotient 
        $$ M_{LC}(X) := M_{LC}^0(X)/\overline{\{0\}}$$
    of $M_{LC}^0$. We denote the natural continuous injection $X\to M_{LC}^0(X)$ by $\gamma_0$ and the natural map $X\to M_{LC}(X)$ by $\gamma$.
\end{defn}

This satisfies the expected universal property:

\begin{prop}[Universal property of $M_{LC}^0$]
    Let $X$ be a topological space. Then, given any continuous map $f:X\to E$ from $X$ to some not-necessarily-Hausdorff locally convex topological vector space $E$, there is a unique continuous linear map $\overline{f}:M_{LC}^0(X) \to E$ making the following diagram commute
    % https://q.uiver.app/?q=WzAsMyxbMCwwLCJYIl0sWzEsMCwiRSJdLFswLDEsIk1fe0xDfShYKSJdLFswLDEsImYiXSxbMCwyLCJcXGdhbW1hIiwyXSxbMiwxLCJcXG92ZXJsaW5le2Z9IiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
    \[\begin{tikzcd}
	X & E \\
	{M_{LC}^0(X)}
	\arrow["f", from=1-1, to=1-2]
	\arrow["\gamma_0"', from=1-1, to=2-1]
	\arrow["{\overline{f}}"', dashed, from=2-1, to=1-2]
    \end{tikzcd}\]
\end{prop}
\begin{proof}
    Since the underlying (algebraic) vector space of $M_{LC}^0(X)$ is the free vector space on $X$, there is a unique linear (\emph{a priori} not-necessarily-continuous) map $\overline{f}$ making the above diagram commute. We need to show that $\overline{f}$ is continuous. But this is evident from the fact that for every seminorm $p$ of $E$,  
        $$\|\cdot\|:= p(\overline{f}(\cdot))$$ 
    is a seminorm on $M_{LC}^0(X)$ such that 
        $$ (x,y)\mapsto \|x-y\|= p(\overline{f}(x-y))= p(f(x)-f(y)) $$
    is continuous on $X\times_{\topsp} X$.
\end{proof}

From the universal properties of $M_{LC}^0$ and the Hausdorff quotient, we immediately obtain:

\begin{prop}[Universal property of $M_{LC}$]\label{uniprop_M_lc}
    Let $X$ be a topological space. Then given any continuous map $f:X\to E$ from $X$ to some \emph{(Hausdorff)} LCTVS $E$, there is a unique continuous linear map $\overline{f}:M_{LC}(X) \to E$ making the following diagram commute:
    \[\begin{tikzcd}
	X & E \\
	{M_{LC}(X)}
	\arrow["f", from=1-1, to=1-2]
	\arrow["\gamma"', from=1-1, to=2-1]
	\arrow["{\overline{f}}"', dashed, from=2-1, to=1-2]
    \end{tikzcd}\]
    (Where $\gamma: X \to M_{LC}(X)$ is the natural map.)
\end{prop}

This also entails the adjunction mentioned in the beginning of the section.

\begin{cor}[The adjunction $M_{LC} \dashv k$]
    Let $X$ be a $k$-space. Then, for any continuous map $f:X\to kE$ from $X$ to the ``underlying $k$-space'' $kE$ of an LCTVS $E$, there is a unique continuous linear map $\overline{f}:M_{LC}(X) \to E$ making the following diagram commute:
    \[\begin{tikzcd}
	X & E \\
	{M_{LC}(X)}
	\arrow["f", from=1-1, to=1-2]
	\arrow["\gamma"', from=1-1, to=2-1]
	\arrow["{\overline{f}}"', dashed, from=2-1, to=1-2]
    \end{tikzcd}\]
    We therefore have an adjunction,
        $$ \hom_{\spaces}(X, kE) \cong \hom_{\lctvs}(M_{LC}(X), E).$$
\end{cor}
\begin{proof}
    Since $f$ is continuous as a map $X\to kE$, it is also continuous as a map $X \to E$ (compose $f$ with the natural map $kE\to E$ which is the identity on the underlying sets). Applying \cref{uniprop_M_lc} to this map $X\to E$ yields the claim.
\end{proof}

\subsection{\texorpdfstring{$\mnd$ is the repleted, $k$-ified free LCTVS}{Mc is the repleted, k-ified free LCTVS}}

The final claim made in the introductory remarks to this section, completing the picture, was the following:

\begin{prop}
    (( Warning : this might actually be wrong )) 
    We have a natural isomorphism,
        $$ \mnd(X) \cong \scompl (k M_{LC}(X)). \hfill (X\in \spaces) $$
\end{prop}
\begin{proof}
    Since the functor $\mnd: \spaces \to \sclin$ is left adjoint to the forgetful functor $\sclin \to \spaces$ and left adjoints are essentially unique, it suffices to show that 
        $$ \scompl \circ k \circ M_{LC}: \spaces \to \sclin $$
    is also left adjoint to the forgetful functor. \par 
    (( no longer sure that what follows can actually be modufied to make sense, since $k$-saturated LCTVS form a \emph{coreflective} subcategory of LCTVS...)) \par
    By the equivalence between the category $\klctvs$ of $k$-locally convex linear $k$-spaces and the category $\mathscr{l}k\lctvs$ of $k$-saturated LCTVS, $k M_{LC}$ is left adjoint to the forgetful functor 
            $$k: \klctvs \to \spaces.$$ 
Moreover, the repletion function $\scompl$ is left adjoint to the inclusion 
    $$k\lctvs \to \sclin. $$
The situation is summarised in the following diagram. 
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJrXFxsY3R2cyJdLFsxLDAsIlxcbWF0aHNjcntsfWtcXGxjdHZzIl0sWzAsMSwiXFxzY2xpbiJdLFsxLDEsIlxcc3BhY2VzIl0sWzAsMSwiXFxzaW0iLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDIsIk0iLDAseyJvZmZzZXQiOi0yfV0sWzAsMiwiXFxzY29tcGwiLDIseyJvZmZzZXQiOjJ9XSxbMSwzLCJrIiwwLHsib2Zmc2V0IjotMn1dLFszLDEsIk1fe0xDfSIsMCx7Im9mZnNldCI6LTJ9XSxbMiwwLCIiLDEseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoiYm90dG9tIn19fV0sWzIsMywiIiwxLHsib2Zmc2V0IjotMX1dLFs1LDEwLCIiLDEseyJsZXZlbCI6MSwic3R5bGUiOnsibmFtZSI6ImFkanVuY3Rpb24ifX1dLFs4LDcsIiIsMix7ImxldmVsIjoxLCJzdHlsZSI6eyJuYW1lIjoiYWRqdW5jdGlvbiJ9fV0sWzYsOSwiIiwxLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XV0=
\[\begin{tikzcd}
	k\lctvs & {\mathscr{l}k\lctvs} \\
	\sclin & \spaces
	\arrow["\sim", Rightarrow, no head, from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "M", shift left=2, from=2-2, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "\scompl"', shift right=2, from=1-1, to=2-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, "k", shift left=2, from=1-2, to=2-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{M_{LC}}", shift left=2, from=2-2, to=1-2]
	\arrow[""{name=4, anchor=center, inner sep=0}, shift right=2, hook', from=2-1, to=1-1]
	\arrow[""{name=5, anchor=center, inner sep=0}, shift left=1, from=2-1, to=2-2]
	\arrow["\dashv"{anchor=center, rotate=90}, draw=none, from=0, to=5]
	\arrow["\dashv"{anchor=center}, draw=none, from=3, to=2]
	\arrow["\dashv"{anchor=center}, draw=none, from=1, to=4]
\end{tikzcd}\]
We conclude that $\scompl k M_{LC}$ is left adjoint to the forgetful functor $\sclin \to \spaces$, as is $M$, whereby the claim follows from the essential uniqueness of adjoints.
\end{proof}


\section{Old section on sequential completeness of $\mnd$-modules}

\subsection{Sequential completeness of $\mnd$-modules}

The following shows that $\mnd$-modules, even though we do not know whether they are $k$-locally convex and $k$-complete in general, do satisfy a milder completeness condition.
 
\begin{prop}\label{seq_compl_M_mods}
    Let $V$ be an $\mnd$-module. Then $V$ is sequentially complete, i.e. every Cauchy sequence in $V$ converges.
\end{prop}
\begin{proof}
    Let $(x_n)$ be a Cauchy sequence in $V$. To show that $(x_n)$ converges, it suffices to prove that $(\delta_{x_n})$ converges in $MV$, since $\delta_\bullet: V \to MV$ is a closed embedding. \par
    To see this, recall that the convergent sequences in a topological space coincide with those of its $k$-ification  and that $\cco(C(V))$ is complete (due to the fact that $C(V)$ is a $k$-space, see \cite[p. 231]{kelley2017general}). Hence, it is indeed sufficient to show that $(\delta_{x_n})$ is a Cauchy sequence in $\cco(C(V))$, since then it converges in $\cco(C(V))$ and therefore equivalently in $C(C(V))$ and $MV$ (because $MV\subseteq C(V)^\wedge \subseteq C(C(V))$ is closed, by definition). \par
    To this end, let $K\subseteq C(V)$ be compact and let $\epsilon>0$. Then $K$ is equicontinuous on each compact subset of $V$ (see \cite[p. 234, Theorem 18]{kelley2017general}). In particular, $K$ is equicontinuous on
        $$ D := \{0\} \cup \{x_n-x_m \in V \mid n,m\in \nats \}, $$
    so there exists a neighbourhood $U$ of the origin in $V$ such that for all $x,y\in U\cap D$ and every $f\in K$,
        $$ |f(x)-f(y)|<\epsilon. $$
    The fact that $(x_n)$ is a Cauchy sequence allows us to choose $N\in \nats$ such that for all $n,m\geq N$, $x_n-x_m\in U$. Now, for every $n,m \geq N$, we have that $x_n,x_m\in x_N + U$ and hence that 
    \begin{align*}
            \|\delta_{x_n}-\delta_{x_m}\|_K 
        &=  \sup_{f\in K} |\delta_{x_n}(f)-\delta_{x_m}(f)| \\
        &=  \sup_{f\in K} |f(x_n)-f(x_m)| < \epsilon.
    \end{align*}
    Therefore, $(\delta_{x_n})$ is a Cauchy sequence in $\cco(C(X))$, completing the proof.
\end{proof}

\begin{example}\label{example_seq_compl_M_mods}
    Let $V$ be any normed space that is not complete (equivalently, not sequentially complete), understood as a linear $k$-space. Then $V$ is not an $\mnd$-module by Proposition \ref{seq_compl_M_mods}. 
\end{example}

\section{Old section on replete linear $hk$-spaces}

\subsection{The repletion of a linear $k$-space.}

Every linear $k$-space can be \emph{repleted}, in a natural way.

\begin{defn}\label{defn_repletion}
    Let $V$ be a linear $k$-space.
    \begin{enumerate}
        \item The \emph{repletion} of $V$, which we denote by $\scompl V$, is the closure of the image of $V$ in $\chi$ under the canonical map $\eta^V: V \to \chi$. Denote the co-restriction of $\eta^V$ to $\scompl V$ by
        	$$ i^V : V \to \scompl V. $$
        \item If $f:V\to W$ is a continuous linear map to another linear $k$-space $W$, we define
            $$ \scompl f: \scompl V \to \scompl W $$
        as the restriction of the ``double adjoint'',
            $$ f^{\wedge\wedge}: \chi \to W^{\wedge\wedge}, \;\;\; \chi \mapsto (\phi \mapsto \chi(\phi \circ f))$$
        to $\scompl V$. (We will show below in lemma \ref{sep_compl_lem} that this is well-defined, i.e. that it does map to $\scompl W$.) Hence, we obtain the \emph{repletion functor} 
            $$ \scompl: \vect \to \sclin, \;\;\; V \to \scompl V, \;\; f\to \scompl f. $$
    \end{enumerate}
\end{defn}

\begin{lem}\label{sep_compl_lem}
    Let $V,W$ be linear $k$-spaces and $f:V\to W$ be a continuous linear map. Then $\scompl f$ is well-defined in that its image is contained in $\scompl W$.
\end{lem}
\begin{proof}
    First, let $\chi=\eta(x)\in \scompl V$, for some $x\in V$. Then 
        $$ (\scompl f) (\chi) = (\scompl f) (\eta(x)) = (\phi \mapsto \eta(x)(\phi \circ f)) = (\phi \mapsto \phi (f(x))) = \eta(f(x)). $$
    Hence, $(\scompl f) (\eta(V)) \subseteq \eta(W)$ and by continuity of $\scompl f$,
        $$ (\scompl f) (\overline{\eta(V)}) \subseteq \overline{(\scompl f) (\eta(V))} \subseteq \overline{\eta(W)} = \scompl W,$$
    showing the claim.
\end{proof}

(( ADD : remark that this construction is similar to one by L. Nel in the context of convergence vector spaces ))

\begin{remark}\label{naturality_of_iV}
    By naturality of $\eta$, we immediately obtain that its co-restriction to $\scompl$, 
        $$ i^V : V \to \scompl V $$
    is a natural transformation, as well. We will show in proposition \ref{uni_prop_scompl} that this natural transformation is indeed the unit of an adjunction between the forgetful functor 
        $$ \sclin \to \vect $$
    and the repletion functor, displaying $\sclin$ as a reflective subcategory of $\vect$ and thus justifying the suggestive terminology ``repletion''. Before we come to that, we need to show that replete linear $k$-spaces are closed under taking closed subspaces.
\end{remark}

\subsection{Closed linear subspaces of replete spaces are replete.}

\begin{prop}\label{cl_sub_scompl_scompl}
	Let $V$ be a replete linear $k$-space and let $W$ be a closed linear subspace. Then $W$ is again replete. 
\end{prop}
\begin{proof}
	Let $\iota: W \to V$ be the inclusion map and let $r^V$ be the inverse of the natural map 
	$$i^V:V \to \scompl V,$$
    which is an isomorphism, as $V$ is assumed to be replete. By naturality of $i^V$ (remark \ref{naturality_of_iV}), represented by the diagram 
		\[\begin{tikzcd}
	    V & {\scompl V} \\
	   W & {\scompl W}
	   \arrow["{i^V}", from=1-1, to=1-2]
	   \arrow["{i^W}"', from=2-1, to=2-2]
	   \arrow["\iota", from=2-1, to=1-1]
	   \arrow["{\scompl \iota}"', from=2-2, to=1-2]
        \end{tikzcd}\]
	we have that $i^V\circ \iota = (\scompl\iota) \circ i^W$. Letting $\tilde{r}^W:=r^V\circ (\scompl \iota)$, this implies that 
		$$ \tilde{r}^W \circ i^W =  r^V\circ (\scompl\iota) \circ i^W = r^V \circ i^V\circ \iota = \iota. $$
    From this, we obtain that the image of $\tilde{r}^W$ is contained in $W$:
    \begin{align*}
	   \tilde{r}^W(\scompl W) = \tilde{r}^W(\overline{i^W(W)} \subseteq \overline{\tilde{r}^W(i^W(W)} = \overline{\iota(W)} = W.
    \end{align*}
    Now, let 
	   $$r^W: cW \to W $$
    be the co-restriction of $\tilde{r}^W$ onto $W$. Then $r^W\circ i^W= \id_W$, so $i^W$ is a split monomorphism and therefore a closed embedding. This proves the claim.
\end{proof}

\subsection{Universal property of repletion}

The repletion satisfies the properties that one would expect of such a construction:

\begin{prop}[Universal property of repletion]\label{uni_prop_scompl}
    Let $V$ be a linear $k$-space. Then 
    \begin{enumerate}[1.]
    	\item $V$ is replete if, and only if,
    		$i^V: V \to \scompl V$
    	is an isomorphism. 
        \item The natural map 
        	$$i^{\scompl V}: \scompl V \to \scompl \scompl V$$
        	is an isomorphism, i.e. the repletion of $V$ is replete.
        \item If $f:V \to W$ is a continuous linear map to some replete linear $k$-space $W$, then there exists a unique continuous linear map $\overline{f}: \scompl V \to W$ such that the following diagram commutes:
            \[\begin{tikzcd}
	        {\scompl V} \\
	        V & W
	       \arrow["f"', from=2-1, to=2-2]
	       \arrow["{i^V}", from=2-1, to=1-1]
	       \arrow["{\overline{f}}", from=1-1, to=2-2]
            \end{tikzcd}\]
        Hence, the repletion functor $\scompl$ is left adjoint to the inclusion functor
            $$  \sclin \hookrightarrow \vect. $$
        \item Moreover, this adjunction is ``enriched'', in that we have a natural isomorphism of linear $k$-spaces:
            $$ \overline{\,\cdot\,}: \:L(\scompl V,W) \cong L(V, W), \;\;\; f \mapsto \overline{f}. $$
        \end{enumerate}
\end{prop}
\begin{proof}
    \begin{enumerate}[1.]
    	\item This is clear.
        \item By proposition \ref{cl_sub_scompl_scompl}, a closed subspace of a replete space is replete. Since $\scompl V \subseteq \chi$ and $\chi$ is replete by proposition \ref{duals_scompl}, this implies that $\scompl V$ is replete.
        \item Since $W$ is replete, $i^W$ is an isomorphism. Let $r^W$ denote its inverse and define
        	$$\overline{f}:= r^W \circ \scompl f : \scompl V \to W$$
        Then by naturality of $i$, $i^W \circ f = \scompl f \circ i^V$ and hence, 
            $$ f = r^W \circ i^W \circ f = r^W \circ \scompl f \circ i^V  = \overline{f} \circ i^V, $$
        showing that the required diagram commutes. To see that $\overline{f}$ is unique with this property, suppose that $\tilde{f} \circ i^V = f$, as well. Then $\tilde{f} \circ i^V = \overline{f} \circ i^V$ and since $i^V$ has dense image and $\scompl V$ is $k$-Hausdorff (by proposition \ref{perm_prop_haus}), this implies $\tilde{f} = \overline{f}$ by lemma \ref{epis_in_lin_k_hausdorff_spaces}.
        \item By cartesian closure of $\spaces$, the map $f \to \overline{f}$ is continuous, with continuous inverse given by $g \mapsto g \circ i^V$. Therefore, the map $f \to \overline{f}$ (which is clearly also linear) is a homeomorphism, as claimed.
    \end{enumerate}
\end{proof}

\begin{cor}
    The category $\sclin$ of replete linear $k$-spaces has all limits and colimits. Limits (in particular products and kernels) are formed as in $\vect$ and colimits (in particular cokernels) are obtained as the repletion of the corresponding colimit in $\vect$.
\end{cor}
\begin{proof}
    It follows directly from proposition \ref{uni_prop_scompl}, that 
        $$ \scompl: \vect \to \sclin $$
    turns $\sclin$ into a reflective subcategory of $\vect$. We have seen that $\vect$ has all limits and colimits (corollary \ref{vect_cocomplete_complete}), and reflective subcategories  inherit (co-)limits in the fashion described (see \cite[p. 142, Proposition 4.5.15]{riehl2017category}).
\end{proof}


\subsection{The natural dual of $\mnd X$ of $CX$}

(( ADD : interpretation of result, c.f. converse Riesz theorem; emphasise use of ``monadic integration calculus'')

\begin{lem}\label{dual_of_MX}
    The natural continuous linear maps
        $$ \theta: \mnd(X)^\wedge \to CX, \;\;\; F \mapsto (x\mapsto F(\delta_x))$$
    and 
        $$ \eta: CX \to \mnd(X)^\wedge, \;\;\; f \mapsto (\mu \mapsto \mu(f))$$
    are mutually inverse and hence constitute natural isomorphisms:
        $$ \mnd(X)^\wedge \cong CX.$$
\end{lem}
\begin{proof}
    We calculate, for any $f\in CX$, $x\in X$,
    \begin{align*}
        \theta \circ \eta (f)(x) &= \theta(\mu \mapsto \mu(f))(x)\\
        &= (\mu \mapsto \mu(f))(\delta_x)\\
        &= \delta_x(f) = f(x) = \id_{CX}(f)(x).
    \end{align*}
    Similarly, for all $F \in \mnd(X)^\wedge$, $\mu \in \mnd X$,
    \begin{align*}
        \eta \circ \theta (F)(\mu) 
        &= \eta(x\mapsto F(\delta_x))(\mu)\\
        &= \mu(x\mapsto F(\delta_x))\\
        &= \int \:F(\delta_x) \,\diff \mu(x) \\
        &= F \Big( \int \,\delta_x \diff \mu(x) \Big) \\
        &= F(\mu) = \id_{\mnd(X)^\wedge}(F)(\mu),
    \end{align*}
    where we have used that $F$ is a continuous linear map in going from the third to the fourth line.
\end{proof}

\begin{cor}\label{CX_sep_compl}
    For every $k$-space $X$, $CX$ is replete.
\end{cor}
\begin{proof}
    This follows from lemma \ref{dual_of_MX} and the fact that the natural of any linear $k$-space is replete (lemma \ref{duals_scompl}).
\end{proof}

\subsection{$\mnd X$ is the free replete linear $k$-space}

\begin{prop}\label{MX_free_sep_compl_lin_space}
    Let $X$ be a $k$-space. Then:
    \begin{enumerate}
        \item $\mnd X$ is a replete linear $k$-space.
        \item For every continuous map $f:X\to V$, with $V$ a replete linear $k$-space, there is a unique continuous linear map $\overline{f}: \mnd X \to V$ such that the following diagram commutes:
        % https://q.uiver.app/?q=WzAsMyxbMCwwLCJYIl0sWzEsMCwiViJdLFswLDEsIlxcbW5kIFgiXSxbMCwxLCJmIl0sWzAsMiwiXFxkZWx0YV9cXGJ1bGxldCIsMl0sWzIsMSwiXFxvdmVybGluZXtmfSIsMl1d
        \[\begin{tikzcd}
	       X & V \\
	       {\mnd X}
	       \arrow["f", from=1-1, to=1-2]
	       \arrow["{\delta_\bullet}"', from=1-1, to=2-1]
	       \arrow["{\overline{f}}"', from=2-1, to=1-2]
        \end{tikzcd}\]
        In other words, we have an adjunction,
            $$ \hom_{\spaces}(X, V) \cong \hom_{\sclin}(MX, V), $$
        exhibiting $M$ as left adjoint to the forgetful functor $\sclin \to \spaces$.
    \end{enumerate}
\end{prop}
\begin{proof}
    \begin{enumerate}
        \item This follows the fact that closed subspaces of replete linear $k$-spaces are again replete (proposition \ref{cl_sub_scompl_scompl}), since $MX$ is a closed subspace of $CCX$ (which is replete by lemma \ref{CX_sep_compl}).
        \item This follows from the fact that replete linear $k$-spaces are $M$-modules and the fact that $MX$ is the free $M$-module on $X$ (lemma \ref{univ_prop_free_T_modules}). 
    \end{enumerate}
\end{proof}

\section{Old section on finite-dimensional linear $hk$-space}



The following facts are well-known for the case of Hausdorff topological vector spaces. Albeit their proofs are the same as in the classical case (which comes down to the fact that the products of $\top$ and $\topsp$ agree in the case of $\mathbb{K}\times V$ by local compactness of $V$ (( TODO : reformulate))), let us record them here for the sake of completeness. (( TODO : maybe readers won't know that anyway; don't be afraid to do ``trivial'' things! )) 

\begin{lem}\label{lem_fctl_continuous_iff_closed_kernel}
    Let $V$ be a linear $hk$-space and let $\phi:V \to \mathbb{K}$ be a linear map, not assumed to be continuous. Then $\phi$ is continuous if, and only if, its kernel $\ker \phi$ is closed.
\end{lem}
\begin{proof}
    (( TODO ))
\end{proof}

\begin{prop}\label{prop_fin_dim_iso_to_Kn}
    Let $V$ be a $n$-dimensional linear $hk$-space with basis $e_1, \dots, e_n$. Then
        $$ \Phi: \mathbb{K}^n \to V, \;\; x \mapsto \sum_{i=1}^n x_i \cdot e_i $$
    is an isomorphism of linear $k$-spaces (i.e. a linear homeomorphism). Consequently, every finite-dimensional linear $hk$-space is isomorphic to $\mathbb{K}^n$ (for some $n\in \mathbb{N}$). 
\end{prop}
\begin{proof}
    Being a composite of continuous maps, it is clear that $\Phi$ is continuous. It is bijective by virtue of basic linear algebra and its inverse is continuous because each composite $\pi_i \circ \Phi^{-1}$ (with $\pi_i: \mathbb{K}^n \to \mathbb{K}$ the canonical projection and $i\in\{1, \dots, n\}$) is a linear functional with closed kernel (an $n-1$-dimensional subspace of $\mathbb{K}^n$) and hence continuous (by lemma \ref{lem_fctl_continuous_iff_closed_kernel}).
\end{proof}

\begin{cor}
    Let $V$ be a linear $k$-space. If $W$ is a finite-dimensional linear $hk$-space, then every linear map $W\to V$ is continuous.
\end{cor}
\begin{proof}
    (( TODO : optional statement; prove if time ))
\end{proof}

\begin{lem}\label{locally_compact_subsp_closed}
    Let $V$ be a linear $k$-space and suppose that $W\subseteq V$ is a linear subspace which is locally compact in the $k$-subspace topology (see Definition \ref{}). Then $W$ is closed in $V$. (( TODO : add ref ))
\end{lem}
\begin{proof}
    (( TODO ))
\end{proof}

\begin{cor}
    Let $V$ be a linear $hk$-space, let $W$ be a finite-dimensional linear $hk$-space and let $f:W \to V$ be an injective linear map. Then $f$ is a closed embedding.
\end{cor}
\begin{proof}
    The image $\im f\subseteq V$ of $f$, topologised as a $k$-subspace of $V$, is a finite-dimensional linear $hk$-space and hence isomorphic to $\mathbb{K}^n$ (for some $n\in\mathbb{N}$, by proposition \ref{prop_fin_dim_iso_to_Kn}). It follows that $f$ is a $k$-embedding and it remains to show that $\im f\subseteq V$ is closed. Since $\mathbb{K}^n$ is locally compact Hausdorff, the image $\im f$ is, too, and therefore, it is closed in $V$ by lemma \ref{locally_compact_subsp_closed}.
\end{proof}

\begin{prop}
    Let $V$ be a locally compact Hausdorff linear $k$-space. Then $V$ is finite-dimensional.
\end{prop}
\begin{proof}
    Since locally compact Hausdorff spaces are $k$-spaces and the product $V\times V$ agrees with the product in $\topsp$, $V$ is a Hausdorff topological vector space. Hence, the claim reduces to a well-known fact (see, for example, \cite[p. 23, 3.6 Theorem]{schaefer1971topological}). 
\end{proof}
\section{Old section on paired linear $hk$-spaces}

\subsection{Paired Linear $hk$-Spaces}

We will now consider two equivalent definitions: that of a \emph{dual pair of linear $k$-Hausdorff spaces}, which will simply be an object of 
$$ \mathsf{chu}_{\mathbb{K}}(\hvect), $$
and that of a \emph{paired linear $k$-space}. While the first one, being an instance of the extensional-separated Chu construction, immediately yields the excellent properties of the resulting category, the second one is much shorter and emphasises that we can view paired linear $k$-spaces as $k$-spaces with additional structure. \par 
Moreover, we will see that this additional structure (in contrast to the case of algebraic dual pairs) is rather subtle and really does not add much in many cases. For example, a Fréchet space can be viewed as a paired linear $k$-space, \emph{in a unique way} (this will be proposition \ref{Frechet_space_paired_linear_k_space_in_unique_way}). 
In light of this observation, and the results of chapter \ref{chapter_comp_to_locally_conv}, paired linear $k$-spaces could be seen as a categorically well-behaved analogue of locally convex topological vector spaces (TVS). That is, in addition to the direct analogy,
$$ \text{algebraic dual pairs  :  sets} \;\; :: \;\; \text{paired linear }k\text{-spaces  : }k\text{-Hausdorff spaces}, $$
we also have the looser analogy,
$$ \text{locally convex TVS  :   topological spaces} \;\; :: \;\; \text{paired linear } k\text{-spaces  : }k\text{-spaces}. $$
Let us first spell out the definition of a dual pair of linear $k$-Hausdorff spaces in detail.

\begin{defn}[Dual pair of linear $k$-Hausdorff spaces]\label{defn_star_linear_spaces}
    We call an object of 
        $$\plin := \mathsf{chu}_{\mathbb{K}}(\hvect)$$ 
    a \emph{dual pair of linear $k$-Hausdorff spaces}. In detail, this means:
    \begin{enumerate}
        \item A \emph{dual pair linear $k$-space} consists of a pair of linear $k$-Hausdorff spaces, 
        \begin{enumerate}
            \item $V$ (the \emph{underlying linear $k$-space, or, space of vectors}) and,
            \item $V^\top$ (the \emph{co-underlying linear $k$-space, or, space of co-vectors}),
        \end{enumerate}
        together with a continuous linear map 
        $$ \langle - , - \rangle : V \times V^\top \to \mathbb{K} $$
        such that the maps 
        $$ V \to (V^\top)^\wedge, \;\;\; x \mapsto \langle x, \,\cdot \,\rangle, $$
        $$ V^\top \to V^\wedge, \;\;\; \phi \mapsto \langle \,\cdot\,, \phi \rangle, $$
        are closed embeddings. (Recall that regular monomorphisms in $\khaus$ and hence in $\hvect$ are given by linear closed embeddings, see proposition \ref{khaus_morphisms}.)
        \item A \emph{morphism of dual pairs of linear $k$-spaces} $V,W$ is a continuous linear map, 
        $$f:V \to W, $$ 
        together with a further continuous linear map,   
        $$f^\top : W^\top \to V^\top, $$
        the \emph{adjoint}, such that for all $x\in V, \phi \in W^\top$,
        $$ \langle f(x), \phi \rangle = \langle x, f^\top(\phi)\rangle. $$
    \end{enumerate}
\end{defn}

If, given a dual pair $(V,V^\top, \langle-,-\rangle)$ of $k$-Hausdorff spaces, we identify $V^\top$ with its image in $V^\wedge$ and remember that a closed subspace of a $k$-Hausdorff is still $k$-Hausdorff, this definition becomes:

\begin{defn}[Paired linear $k$-space]
    A \emph{paired linear $k$-space} is a linear $k$-space $V$ together with a closed linear subspace $V^\top \subseteq V^\wedge$ of its dual, such that the map 
        $$ V \to (V^\top)^\wedge, \;\;\; x \to (\phi \mapsto \phi(x)), $$
    is a closed embedding. A morphism of paired linear $k$-spaces $V, W$, or \emph{paired linear map}, is a linear map $f:V\to W$ such that 
        $$ f^\wedge(W^\top) \subseteq V^\top. $$
\end{defn}

We will loosely identify these two notions and write ``paired linear $k$-space'' also for what would strictly have to be called a dual pair of linear $k$-Hausdorff spaces. Accordingly, $\plin$ will also be our notation for the category of paired linear $k$-spaces. 

\subsection{Paired linear $k$-spaces form a bicomplete $*$-autonomous category over $\khaus$.} 

Applying theorem \ref{construction_thm_for_star_aut_cats_over_cccs}, we immediately obtain:

\begin{thm}\label{paired_lin_k_spaces_star_aut}
    The category $\plin$ of paired linear $k$-spaces is a bicomplete $*$-autonomous category over the cartesian closed category $\khaus$ of $k$-Hausdorff spaces. 
\end{thm}

\begin{notation}
    We write $MX$ for the free paired linear $k$-space on a $k$-Hausdorff space $X$, as well as, 
        $$ V \ptimes W := V \otimes_{\plin} W, $$
        $$ V \multimap W := [V, W]_{\plin}, $$
        $$ V^* := V \multimap \mathbb{K}, $$
    for the tensor product, internal hom and dualisation functor of $\plin$, respectively, and 
        $$ C(X, V) := MX \multimap V \cong V^*\multimap C(X),\;\, C(X) := C(X, \mathbb{K}) = (MX)^*, \;\;\;\; (X \in \khaus, V \in \plin)$$
    for the paired linear $k$-space of continuous maps from $X$ to $V$. That the underlying space of vectors of $C(X,V)$ is exactly (naturally homeomorphic to) the $k$-space of continuous maps $V^X$ from $X$ to $V$ follows from the fact that $M$ is left adjoint to the forgetful functor $\plin \to \khaus$. \par 
    Moreover, we denote by 
        $$ V \multimapdot W := V^* \ptimes W $$
    the \emph{matrix-type maps} from $V$ to $W$ (this terminology will be justified later, by proposition \ref{matrix_type_ops_as_plin_maps}), and by
        $$ V \cotimes W := (V^* \ptimes W^*)^*$$
    the \emph{dual tensor product}.
    In addition, we write, 
        $$ M(X,V) :=  CX \multimap V \cong V^* \multimap MX, \;\;\;\; (X \in \khaus, V \in \plin). $$
\end{notation}

We will see in Chapter \ref{chap_mon_for_vv_int}, section \ref{sec_riesz_mark_type_thm}, that the elements of $M(X,V)$ are (in a natural bijection with) compactly supported $V$-valued measures of a specific sort. \par 
All in all, the interpretations of the various constructions that arise from the $*$-autonomous-over-cartesian-closed structure of $\plin$ are summarised in table \ref{table_interpretations_plin}. 

\begin{table}[h]\label{table_interpretations_plin}
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{Functional-Analytic Interpretations of Constructions in $\plin$}}                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{\textit{Paired linear $k$-space of:}}                                                                                 & \multicolumn{1}{c|}{\textit{Given by:}} & \textit{Justification/precise statement:}                                                                                                                                 \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}compactly supported \\ $V$-valued measures on $X$\end{tabular}}                            & \multicolumn{1}{c|}{$M(X,V)$}           & \begin{tabular}[c]{@{}c@{}}(( know this for the case of\\ $V=\mathbb{K}$, see next chapter ))\end{tabular}                                                                \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}$V$-valued continuous \\ functions on $X$\end{tabular}}                                    & \multicolumn{1}{c|}{$C(X,V)$}           & \begin{tabular}[c]{@{}c@{}}definition\\ /tensor-hom adjunction\end{tabular}                                                                                               \\ \hline
\multicolumn{1}{|c|}{paired linear maps $V\to W$}                                                                                   & \multicolumn{1}{c|}{$V \multimap W$}    & definition                                                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{matrix-type maps $V\to W$}                                                                                       & \multicolumn{1}{c|}{$V \multimapdot W$}    & \begin{tabular}[c]{@{}c@{}}(( ... ))\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}compactly supported $V$-valued measures\\ with Radon-Nikodym property on $X$\end{tabular}} & \multicolumn{1}{c|}{$MX \ptimes V$}     & \begin{tabular}[c]{@{}c@{}}(( known for $V$ Banach; need to\\ appropriately define R.-N. property\\ in general case ))\end{tabular}                                       \\ \hline
\end{tabular}
\end{table}

These constructions are interrelated by a number of formulas:

\begin{prop}
    We have the following natural isomorphisms in $\plin$, for any $k$-Hausdorff spaces $X,Y$ and paired linear $k$-spaces $V,W,Z$,
    \begin{align*}
        V \ptimes W \multimap Z &\cong V \multimap (W \multimap Z)
    \end{align*}
    (( FINISH ))
\end{prop}

listed in table \ref{table_interpretations_plin}, all of which follow immediately from applying the tensor-hom adjunction of $\plin$, duality (i.e. $*$-autonomy of $\plin$), cartesian closure of $\khaus$ or, the monoidal free-forgetful adjunction $M \dashv |\cdot|$ between $\plin$ and $\khaus$. 


\subsection{Fréchet and Brauner spaces are paired linear $k$-spaces in a unique way.}

The following proposition shows that every Fréchet space (and every Brauner space likewise) provides an example of a paired linear $k$-space, and that there is no choice in the way it does so.

\begin{prop}\label{Frechet_space_paired_linear_k_space_in_unique_way}
    Let $V$ be a Fréchet space or a Brauner space. Then $V$ becomes a paired linear $k$-space with underlying space of vectors $V$ by letting the co-underlying space of co-vectors be the natural dual,
        $$ V^\top := V^\wedge, $$
    with the pairing $\langle - , - \rangle$ given by the evaluation pairing. Moreover, if $\tilde{V}$ is any other paired linear $k$-space whose underlying space of vectors is $V$, then the identity $V \to \tilde{V}$ is an isomorphism of paired linear $k$-spaces. 
\end{prop}
\begin{proof}
    That $V$ is a paired linear $k$-space in this way follows from Smith duality (\ref{Smith_duality}). \par 
    For the second part of the claim concerning uniqueness, notice that the assumption that
        $$ G: V \to (\tilde{V}^\top)^\wedge, \;\;\;x \mapsto \langle x ,  \rangle $$
    is a closed embedding implies that  
        $$ G^\wedge \circ \eta^{\tilde{V}^\top} : \tilde{V}^\top \to V^\wedge, \;\;\;\phi \mapsto \langle - , \phi \rangle $$
    is surjective, using the Hahn-Banach extension theorem (and Smith duality, once again). Being also a closed embedding by assumption, we see that $G^\wedge \circ \eta^{\tilde{V}^\top}$ is an isomorphism of linear $k$-spaces. Moreover, $G^\wedge \circ \eta^{\tilde{V}^\top}$ is  adjoint to the identity map $V\to \tilde{V}$, thus proving the claim.
\end{proof}


\subsection{The topology of spaces of linear operators}\label{top_on_spc_of_linops}


\subsection{The big picture.} Combining theorem \ref{paired_lin_k_spaces_star_aut} and proposition \ref{Frechet_space_paired_linear_k_space_in_unique_way}, the following picture emerges.

% https://q.uiver.app/?q=WzAsNyxbMSwzLCJcXGtoYXVzIl0sWzAsMiwiXFxwbGluIl0sWzIsMiwiXFxwbGluXlxcb3AiXSxbMCwxLCJcXG1hdGhzZntGcmVlfSJdLFsyLDEsIlxcbWF0aHNme0JyYX1eXFxvcCJdLFsyLDAsIlxcbWF0aHNme1NtaX1eXFxvcCJdLFswLDAsIlxcbWF0aHNme0Jhbn0iXSxbMCwxLCJNKC0pIiwwLHsiY3VydmUiOi0xfV0sWzAsMiwiQygtKSIsMix7ImN1cnZlIjoxfV0sWzMsMSwiIiwxLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbNCwyLCIiLDEseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6ImJvdHRvbSJ9fX1dLFs1LDQsIiIsMSx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoiYm90dG9tIn19fV0sWzYsMywiIiwxLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbMyw0LCIoLSleXFx3ZWRnZSIsMV0sWzEsMiwiKC0pXioiLDFdLFs2LDUsIigtKV5cXHdlZGdlIiwxXSxbMiwwLCIiLDAseyJjdXJ2ZSI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsMCwiIiwxLHsiY3VydmUiOi0xLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNywxNywiIiwwLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XSxbOCwxNiwiIiwyLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XV0=
\[\begin{tikzcd}
	{\mathsf{Ban}} && {\mathsf{Smi}^\op} \\
	{\mathsf{Free}} && {\mathsf{Bra}^\op} \\
	\plin && {\plin^\op} \\
	& \khaus
	\arrow[""{name=0, anchor=center, inner sep=0}, "{M(-)}", curve={height=-6pt}, from=4-2, to=3-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{C(-)}"', curve={height=6pt}, from=4-2, to=3-3]
	\arrow[hook, from=2-1, to=3-1]
	\arrow[hook', from=2-3, to=3-3]
	\arrow[hook', from=1-3, to=2-3]
	\arrow[hook, from=1-1, to=2-1]
	\arrow["{(-)^\wedge}"{description}, from=2-1, to=2-3]
	\arrow["{(-)^*}"{description}, from=3-1, to=3-3]
	\arrow["{(-)^\wedge}"{description}, from=1-1, to=1-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, curve={height=6pt}, dashed, from=3-3, to=4-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, curve={height=-6pt}, dashed, from=3-1, to=4-2]
	\arrow["\dashv"{anchor=center, rotate=31}, draw=none, from=0, to=3]
	\arrow["\dashv"{anchor=center, rotate=154}, draw=none, from=1, to=2]
\end{tikzcd}\]

Here, $\mathsf{Ban}, \mathsf{Smi}, \mathsf{Fré}, \mathsf{Bra}$ denote the categories of Banach(able), Smith, Fréchet and Brauner spaces, respectively. The dashed arrows are the respective forgetful functors assigning to a paired linear $k$-space its (co-)underlying space of (co-)vectors. The other (solid) arrows form a commutative diagram. 

\subsection{The free paired linear $k$-space.}

\subsection{The tensor product and the dual tensor product.}

\subsubsection{Integral representation of tensors.}

\begin{prop}\label{int_rep_tensors_prop}
    (( MISSING : Integral representation of tensors )) 
\end{prop}

\subsubsection{Universal properties.}

\subsubsection{Relation to tensor products of Banach spaces.}

(( MISSING ))

\subsection{Matrix-type maps} 

\subsubsection{Matrix-type maps as paired linear maps with continuous matrix representation}

(( ADD : introductory words ))

\begin{prop}\label{matrix_type_ops_as_plin_maps}
    Let $V,W$ be paired linear $k$-spaces. Then the natural morphism 
        $$ (V \multimapdot W) \to (V \multimap W), \;\;\; \phi \otimes w \mapsto (v \mapsto \phi(v) w $$
    is injective. Hence, using the integral representation (proposition \ref{int_rep_tensors_prop}) of tensors in 
        $$ V \multimapdot W = V^* \ptimes W, $$
    we can identify elements of $V \multimapdot W$ with paired linear maps $V\to W$ that admit a representation of the form 
        $$ V \ni v \mapsto \int \phi(v) w \diff \mu(\phi, w) \in W, $$
    for some $\mu \in M(V^*\times W)$. 
\end{prop}

This is a continuum version of a matrix representation of a linear map, in which the measure $\mu$ takes the place the scalar entries of the matrix. When 
$$\mu := \sum_{i=0}^n \mu_i \delta_{(\phi_i, w_i)}$$
is a finitely supported measure, then expression \ref{} becomes 
$$ ... $$
(( FINISH ))

\subsubsection{Matrix-type maps on Hilbert spaces are trace-class operators}

(( MISSING ))

\subsubsection{The trace of a matrix-type map.}

(( MISSING ))

(( MISSING : polar duality applied to paired linear $k$-spaces; "Akbarov's dictionary" )) 




\section{Planning/To-do}

\begin{itemize}
    \item Paired linear $k$-spaces:
    \begin{itemize}
        \item good name?
        \item relation of tensor product to classical topological tensor products?
        \item trace class operators and trace
        \item dictionary of properties: separable, metrisable, Heine-Borel, ...
        \item algebras: group of units/group algebra adjunction, representations as modules, etc. 
    \end{itemize}
    \item Correct and clean-up section on relation to free LCTVS
    \item Make "conjectural table" on equational theories giving rise to measure monads.
    \item add section discussing Chu-construction and $M$ arising from it.
    \item Add non-examples of $M$-modules, sequential completeness
    \item Add context/remarks to section on $k$-completeness
    \item make Venn diagram summarising relationships.
    \item section on (linear) $k$-spaces:
    \begin{itemize}
        \item correct notation in adjunctions.
        \item proofread. 
    \end{itemize}
    \item Illustrative examples:
    \begin{itemize}
        \item Concerning monadic vector-valued integration: Sum of Dirac deltas at integer-radius circles in $\mathbb{R}^2$ can be represented as an integral with value in space of tempered distribution. Does this or a variation of this example allow for an easier calculation of the Fourier transform than otherwise possible?
        \item Convergence of discrete sums to path length. (As an instance of a more general convergence?) 
    \end{itemize}
    \item story / paradigms:
    \begin{itemize}
        \item ``where does $***$ come from?'' e.g. tensor product come from commutative monads (examples: ordinary tensor product of modules, further algebraic examples, topological/normed tensor products; ``completed'' tensor products come from chu constuction), vector valued integration and its properties come from the fact that linear spaces are modules over a measure monad, ...
        \item ``Vector-valued integration and its properties can be understood and summarised entirely by noting that the vector spaces to be integrated in are modules over a commutative monad of measures. ''
        \item ``Generalised functions are generalised elements''
        \item ...
    \end{itemize}
\end{itemize}

\section{``Big Pictures''}

% https://q.uiver.app/?q=WzAsMTAsWzIsMywiXFxzY2xpbl5cXG9wIl0sWzEsMywiXFxtYXRoc2Z7QnJhfV5cXG9wIl0sWzAsMywiXFxtYXRoc2Z7U21pfV5cXG9wIl0sWzMsMywiXFxiaWxpbl5cXG9wIl0sWzQsMiwiXFxzcGFjZXMiXSxbMywxLCJcXGJpbGluIl0sWzIsMSwiXFxzY2xpbiJdLFsxLDEsIlxcbWF0aHNme0Zyw6l9Il0sWzAsMSwiXFxtYXRoc2Z7QmFufSJdLFsyLDAsIlxcdmVjdCJdLFsyLDEsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoidG9wIn19fV0sWzEsMCwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbMCwzLCIiLDAseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6InRvcCJ9fX1dLFs0LDMsIkMoLSkiXSxbOCw3LCIiLDAseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6InRvcCJ9fX1dLFs3LDYsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoidG9wIn19fV0sWzYsNSwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbOCwyLCJcXDtcXDtcXDsoLSleXFx3ZWRnZSJdLFs3LDEsIlxcO1xcO1xcOygtKV5cXHdlZGdlIl0sWzUsMywiKC0pXipcXDoiLDJdLFs0LDUsIk0iLDJdLFs1LDQsIiIsMix7Im9mZnNldCI6NCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzYsOSwiIiwwLHsib2Zmc2V0IjoyfV0sWzksNiwiIiwyLHsib2Zmc2V0IjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNSw2LCIiLDAseyJvZmZzZXQiOi00LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMywwLCIiLDAseyJvZmZzZXQiOjQsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsyMCwyMSwiIiwwLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XSxbMjMsMjIsIiIsMix7ImxldmVsIjoxLCJzdHlsZSI6eyJuYW1lIjoiYWRqdW5jdGlvbiJ9fV0sWzE2LDI0LCIiLDIseyJsZXZlbCI6MSwic3R5bGUiOnsibmFtZSI6ImFkanVuY3Rpb24ifX1dLFsyNSwxMiwiIiwwLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XV0=
\[\begin{tikzcd}
	&& \vect \\
	{\mathsf{Ban}} & {\mathsf{Fré}} & \sclin & \bilin \\
	&&&& \spaces \\
	{\mathsf{Smi}^\op} & {\mathsf{Bra}^\op} & {\sclin^\op} & {\bilin^\op}
	\arrow[hook, from=4-1, to=4-2]
	\arrow[hook, from=4-2, to=4-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, hook, from=4-3, to=4-4]
	\arrow["{C(-)}", from=3-5, to=4-4]
	\arrow[hook, from=2-1, to=2-2]
	\arrow[hook, from=2-2, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, hook, from=2-3, to=2-4]
	\arrow["{\;\;\;(-)^\wedge}", from=2-1, to=4-1]
	\arrow["{\;\;\;(-)^\wedge}", from=2-2, to=4-2]
	\arrow["{(-)^*\:}"', from=2-4, to=4-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "M"', from=3-5, to=2-4]
	\arrow[""{name=3, anchor=center, inner sep=0}, shift right=4, dashed, from=2-4, to=3-5]
	\arrow[""{name=4, anchor=center, inner sep=0}, shift right=2, from=2-3, to=1-3]
	\arrow[""{name=5, anchor=center, inner sep=0}, shift right=2, dashed, from=1-3, to=2-3]
	\arrow[""{name=6, anchor=center, inner sep=0}, shift left=4, dashed, from=2-4, to=2-3]
	\arrow[""{name=7, anchor=center, inner sep=0}, shift right=4, dashed, from=4-4, to=4-3]
	\arrow["\dashv"{anchor=center, rotate=-127}, draw=none, from=2, to=3]
	\arrow["\dashv"{anchor=center}, draw=none, from=5, to=4]
	\arrow["\dashv"{anchor=center, rotate=-90}, draw=none, from=1, to=6]
	\arrow["\dashv"{anchor=center, rotate=-90}, draw=none, from=7, to=0]
\end{tikzcd}\]


\section{Convenient Measure Monads?}

...

\section{Equational Theories, Tensor Products, Chu Construction}

\begin{prop}
    Let $\mathsf{C}$ be a bi-complete, well-powered, regular cartesian closed category and let $T$ be a commutative equational theory. Then the forgetful functor 
        $$ T\mathsf{Mod}(\mathsf{C}) \to \mathsf{C} $$
    is monadic ((DEFINE THIS)) and the induced strong ((DEFINE THIS)) monad $F_T$ on $\mathsf{C}$ is finitary and commutative (thus endowing  $T\mathsf{Mod}(\mathsf{C})$ with the structure of a closed monoidal category by ((ADD)) ).
\end{prop}

\begin{displaycomment}
    Plan: Split all of these statements into small bits being as precise as possible in the specific statements and make less formal, more readable remarks in introductory paragraph to section. Make graphics about what leads to what: \par 
    1. finitary commutative monad implies co-completeness of E-M category and hence tensors. \par 
    2. finitary commutative theory implies finitary commutative monad
    3. $T$ finitary commutative monad and $R$ \emph{commutative} monoid in $\mathsf{C}^T$ implies $R \otimes T$ commutative monad.
    4. closed monoidal category leads to $*$-autonomous category via $\mathsf{chu}$-construction. 
\end{displaycomment}

\begin{thm}
    Let $\mathsf{C}$ be a bi-complete, well-powered, regular, cartesian closed category and let $T$ be a finitary commutative monad. Then:
    \begin{enumerate}
        \item $(\mathsf{C}^T, \otimes_T, T(1_{\mathsf{C}}))$ is a bi-complete, well-powered, regular closed monoidal category.
        \item If $R$ is any monoid in $(\mathsf{C}^T, \otimes_T, T(*))$, then $R\otimes_T T$ is (( SPECIFY STRUCTURE)) a finitary commutative monad on $\mathsf{C}$ whose modules are precisely the $R$-actions.
    \end{enumerate}
\end{thm}

\begin{cor}
    Let $\mathsf{C}$ be a bi-complete, well-powered, regular cartesian closed category. Then $\mathsf{Ab}(\mathsf{C})$ is a bi-complete, well-powered quasi-abelian category. Moreover, the forgetful functor 
        $$ \mathsf{Ab}(\mathsf{C}) \to \mathsf{C} $$
    is monadic ((DEFINE THIS)) and the induced strong ((DEFINE THIS)) (``free abelian group'') monad $F_{\mathsf{Ab}}$ on $\mathsf{C}$ is commutative, endowing  $\mathsf{Ab}(\mathsf{C})$ with the structure of a closed monoidal category.
\end{cor}



\begin{cor}
    Let $\mathsf{C}$ be a bi-complete, well-powered, regular cartesian closed category, and let $R$ be a ring object. Then $R\mathsf{Mod}(\mathsf{C})$ is a bi-complete, well-powered quasi-abelian category. Furthermore, the forgetful functor 
        $$ R\mathsf{Mod}(\mathsf{C}) \to \mathsf{C} $$
    is monadic ((DEFINE THIS)) and the induced strong ((DEFINE THIS)) (``free abelian group'') monad $F_{R} = R \otimes_{\mathsf{Ab}} F_\mathsf{Ab}$ on $\mathsf{C}$ is commutative, endowing  $R\mathsf{Mod}(\mathsf{C})$ with the structure of a closed monoidal category.
\end{cor}
\begin{proof}
    ...
\end{proof}

\begin{thm}
    Given 
    \begin{enumerate}
        \item a bi-complete, well-powered, regular cartesian closed category $\mathsf{C}$,
        \item a ring object $R$ in $\mathsf{C}$, 
        \item and an $R$-module $D$,
    \end{enumerate}
    the category 
        $$\mathsf{D} := \mathsf{chu}(R\mathsf{Mod}(\mathsf{C}), D)$$ 
    has the following properties:
    \begin{enumerate}
        \item $\mathsf{D}$ is $*$-autonomous.
        \item The forgetful functor 
            $$ U: \mathsf{D} \to \mathsf{C} $$
        is faithful and has a left adjoint
            $$ F_{\mathsf{D}}: \mathsf{C} \to \mathsf{D}, $$
        such that:
        \begin{enumerate}
            \item The induced monad $M_T := U \circ F_T$ is a commutative monad.
            \item The natural map $T \to M_T$ is an epimorphism.
        \end{enumerate}
        \begin{displaycomment}
            \textbf{Question:} Is $\mathsf{chu}(\mathsf{C}^T, D)$ a regular category?
        \end{displaycomment}
    \end{enumerate}
 \end{thm}

 \section{Monoidal Categories and Related Concepts}

 ...

 \section{Applications of $*$-linear/bilinear $k$-spaces: $*$-linear algebras?}

\subsubsection{A Stone-Weierstrass-type theorem}

(( The only closed, point-separating ``$*$-linear subalgebra $A$ of $C(X)$ should be $A=C(X)$, at least when $X$ is ``regular'' in some sense. --> Gelfand-type dualities ?)) 

\subsubsection{The group-of-units-group-algebra adjunction}

\section{Deleted sections on replete spaces etc.}

\subsection{Does every replete linear $k$-space have the extension property?}

\begin{defn}
    Let $V$ be a linear $k$-space. We say that $V$ has the \emph{extension property} if, and only if, for any closed linear subspace $W \subseteq V$ and any continuous linear functional $\phi\in W^\wedge$ on $W$, $\phi$ has an extension $\tilde{\phi}\in V^\wedge$ to all of $V$.
\end{defn}

The following is a lemma in the direction of an answer to the question whether every replete linear $k$-space has the extension property. The idea is that an affirmative answer would mean equivalently that the ground field $\mathbb{K}$ is an injective object in the category of replete linear $k$-spaces. In categories in which the pushout of a (regular) monomorphism is a (regular) monomorphism (whether this holds in $\sclin$ is unclear at the moment), this is in turn equivalent to the assertion that every regular monomorphism $\mathbb{K}\to V$ in $\sclin$ is split, which is true:

\begin{lem}
    Let $V$ be a replete linear $k$-space and let $s:\mathbb{K}\to V$ be an injective continuous linear map. Then there is a continuous linear functional $r:V\to \mathbb{K}$ such that $r\circ s = \id_{\mathbb{K}}$, i.e.~$r$ is a retraction of $s$.
\end{lem}
\begin{proof}
    Since $V$ is replete, the map
        $$ j: V \to C(V^\wedge), \;\;\; x \mapsto (\phi \mapsto \phi(x))$$
    is a closed embedding. Now, the injective continuous linear map $\overline{s}:= j \circ s$, 
        $$ \overline{s}: \mathbb{K} \to C(V^\wedge), $$
    is also continuous when viewed as a map 
        $$ \tilde{s}: \mathbb{K} \to \cco(V^\wedge), $$
    using the adjunction (\ref{kification_adjunction}) and the fact that $\mathbb{K}$ is a $k$-space. $\cco(V^\wedge)$ is a locally convex Hausdorff topological and any injective continuous linear function from the ground field $\mathbb{K}$ to a Hausdorff topological vector space is an embedding. Hence, $\tilde{s}$ is an isomorphism (of topological vector spaces) onto its image $\text{im}(\tilde{s})$. Let 
        $$ \phi: \text{im}(\tilde{s}) \to \mathbb{K}$$
    be its inverse. Then $\phi$ is a continuous linear functional on a subspace of the locally convex Hausdorff topological vector space $\cco(V^\wedge)$. By the Hahn-Banach extension theorem, there exists a functional $\tilde{\phi}$ on all of $\cco(V^\wedge)$ extending $\phi$. Let $\tilde{r}:= k \tilde{\phi}$ be the $k$-ification of $\tilde{\phi}$. Keeping in mind that $k\cco(V^\wedge)=C(V^\wedge)$, this yields a continuous linear functional 
        $$ \tilde{r}: C(V^\wedge) \to \mathbb{K}. $$
    Let $r=\tilde{r}|_V$ be the restriction of $\tilde{r}$ to $V\hookrightarrow C(V^\wedge)$. Then $r:V\to \mathbb{K}$ is the desired linear functional, since for $\lambda \in\mathbb{K}$,
        $$ r \circ s (\lambda)= \tilde{r}(\tilde{s}(\lambda)) = \phi(\tilde{s}(\lambda)) = \lambda. $$
\end{proof}

\section{Sequential completeness of $M$-modules}

\begin{prop}
    Let $V$ be an $M$-module. Then $V$ is sequentially complete, i.e. every Cauchy sequence in $V$ converges.
\end{prop}
\begin{proof}
    Let $(x_n)$ be a Cauchy sequence in $V$. To show that $(x_n)$ converges, it suffices to prove that $(\delta_{x_n})$ converges in $MV$, since $\delta_\bullet: V \to MV$ is a closed embedding. \par
    To see this, recall that the convergent sequences in a topological space coincide with those of its $k$-ification (( ADD REF )) and that $\cco(C(V))$ is complete (( ADD REF )). Hence, it is indeed sufficient to show that $(\delta_{x_n})$ is a Cauchy sequence in $\cco(C(V))$, since then it converges in $\cco(C(V))$ and therefore equivalently in $C(C(V))$ and $MV$ (because $MV\subseteq C(V)^\wedge \subseteq C(C(V))$ is closed, by definition). \par
    To this end, let $n,m\in \nats$, let $K\subseteq C(V)$ be compact and let $\epsilon>0$. The fact that $(x_n)$ is a Cauchy sequence allows us to choose $N\in \nats$ such that for all $n,m\geq N$, $x_n-x_m\in U$. Moreover, since $K\subseteq C(V)$ is compact, it is equicontinuous on each compact subset of $V$ (see \cite[p. 234, Theorem 18]{kelley2017general}. In particular, $K$ is equicontinuous at $x_N$ (( This point of the argument is not valid, ``on each compact subset'' means something else; restrict to some compact subset instead, is that works )), so there exists a neighbourhood $U$ of the origin in $V$ such that for all $x,y\in x_N + U$ and every $f\in K$,
    $$ |f(x)-f(y)|<\epsilon. $$
    Now, for every $n,m \geq N$, we have that $x_n,x_m\in x_N + U$ and hence that 
    \begin{align*}
            \|\delta_{x_n}-\delta_{x_m}\|_K 
        &=  \sup_{f\in K} |\delta_{x_n}(f)-\delta_{x_m}(f)| \\
        &=  \sup_{f\in K} |f(x_n)-f(x_m)| < \epsilon.
    \end{align*}
    Therefore, $(\delta_{x_n})$ is a Cauchy sequence in $\cco(C(X))$, completing the proof.
\end{proof}



\section{Some further lemmas}

\subsection{$k$-Embeddings of separated-complete linear $k$-spaces are closed.}

\begin{lem}
    (( does this work? )) Let $V, W$ be a separated-complete linear $k$-space and let 
        $$ \iota: W \to V$$
    be a linear $k$-embedding. Then $\iota$ is, in fact, a \emph{closed} embedding.
\end{lem}
\begin{proof}
    (( Use that separated completion = closure in double dual ))
\end{proof}

\subsection{One-dimensional subspaces of linear $k$-spaces are split}

\begin{lem}
    Let $V$ be a separated-complete linear $k$-space. Then every one-dimensional subspace $\mathbb{K}v \subseteq V$ (with $v\in V$) of $V$ is split, i.e.~there exists a closed linear subspace $W\subseteq V$ such that 
    \begin{enumerate}[1.]
        \item $W + \mathbb{K}v = V$,
        \item $W \cap \mathbb{K}v = 0$,
        \item The map 
            $$+: W \oplus \mathbb{K}v \to V, \;\;\;(w, \lambda v) \mapsto w+\lambda v$$
        is an isomorphism.
    \end{enumerate}
\end{lem}
\begin{proof}
    Since $V$ is separated-complete, the map
        $$ j: V \to C(V^\wedge), \;\;\; x \mapsto (\phi \mapsto \phi(x))$$
    is a closed embedding. Now, the injective continuous linear map  
        $$ s: \mathbb{K} \to C(V^\wedge), \;\;\; \lambda \mapsto j(\lambda v) $$
    is also continuous when viewed as a map 
        $$ \tilde{s}: \mathbb{K} \to \cco(V^\wedge), $$
    using the adjunction (\ref{kification_adjunction}) and the fact that $\mathbb{K}$ is a $k$-space. $\cco(V^\wedge)$ is a locally convex Hausdorff topological and any injective continuous linear function from the ground field $\mathbb{K}$ to a Hausdorff topological vector space is an embedding. Hence, $\tilde{s}$ is an isomorphism (of topological vector spaces) onto its image $\text{im}(\tilde{s})$. Let 
        $$ \phi: \text{im}(\tilde{s}) \to \mathbb{K}$$
    be its inverse. Then $\phi$ is a continuous linear functional on a subspace of the locally convex Hausdorff topological vector space $\cco(V^\wedge)$. By the Hahn-Banach extension theorem, there exists a functional $\tilde{\phi}$ on all $\cco(V^\wedge)$, extending $\phi$. Let $r:= k \tilde{\phi}$ be the $k$-ification of $\tilde{\phi}$. Keeping in mind that $k\cco(V^\wedge)=C(V^\wedge)$, this yields a continuous linear functional 
        $$ r: C(V^\wedge) \to \mathbb{K}, $$
    satisfying $r \circ s = \id_{\mathbb{K}}$, since
        $$ r \circ s (\lambda)= r(\tilde{s}(\lambda)) = \phi(\tilde{s}(\lambda)) = \lambda. $$
    Let $W= \ker r$ be the kernel of $r$. Then:
    \begin{enumerate}[1.]
        \item $W + \mathbb{K}v = V$, since $r(x-r(x)v)= 0$, so $x-r(x)v \in \ker r = W$, for all $x\in V$.
        \item $W \cap \mathbb{K}v = 0$: if $w=\lambda v \in W \cap \mathbb{K}v$ $\lambda r(v) = r(w) = 0$ implies that $\lambda=0$, hence $w=0$.
        \item \item The map 
            $$+: W \oplus \mathbb{K}v \to V, \;\;\; (w, \lambda v) \mapsto w+\lambda v$$
        has an inverse, given by 
            $$ (\id_V-r) \oplus r: V \to W \oplus \mathbb{K}v, \;\;\; x \mapsto (\id_V-r(x), r(x)), $$
        since 
            $$ + \circ ((\id_V-r) \oplus r) = \id_V, $$
        and
            $$ ((\id_V-r) \oplus r) \circ + (w, \lambda v) = (w + \lambda v - r(w + \lambda v), r(w + \lambda v))= (w, \lambda v), $$
        for all $w\in w$, $\lambda \in \mathbb{K}$.
    \end{enumerate}
\end{proof}

\subsection{A Hahn-Banach-type extension principle}

\begin{lem}[One-dimensional extension lemma]
    Let $W\subseteq V$ be a closed linear subspace of some separated-complete linear $k$-space $V$, let $\phi\in W^\wedge$ be a continuous linear functional, and let  $v\in V$. Then there is an extension
        $$ \tilde{\phi}: W + \mathbb{K}v \to \mathbb{K} $$
    of $\phi$ to $W + \mathbb{K}v$. 
\end{lem}
\begin{proof}
    ( THIS IS NOT THE MOST STRAIGHTFORWARD THING TO TRY AND MIGHT NOT WORK ) Assume without loss of generality that $v\not\in W$ (otherwise, there is nothing to show), i.e.~that $W\cap \mathbb{K}v = 0$. 
\end{proof}











\section{Further examples of monads}

\subsection{Algebraic theories and their (Lawvere) syntactic categories}

\begin{example}[Term algebra monad]
    Let $S:=\{f,g,...\}$ be a finite set of ``function symbols'' and let 
        $$ \mathsf{arity}: S \to \nats $$
    be a map, thought of as specifying number of inputs of each would-be function in $S$. For any set $X$, we can define the \emph{term algebra} $TX$ on $X$ for the \emph{signature} $(S,\mathsf{arity})$ as inductively as follows.
    \begin{enumerate}
        \item Each element of $X$, thought of as an ``abstract variable'', defines an element of $TX$ (a ``term'').
        \item Each function symbol $F\in S$ and any sequence $t_1, t_2, ... \in TX$ of terms with length $\mathsf{arity}(F)$ defines an element of $TX$, written $F(x_1, x_2, ..)$.
    \end{enumerate}
    Now, given a fixed set of variables $A$ and set of pairs $E\subseteq TA\times TA$ (thought of as ``equations''), ... \\
    (( Maybe it would be nice to introduce algebraic theories in an appendix? This is leading to far here, though. ))
\end{example}

\subsection{Double dualisation monads}

\begin{example}[Double dualisation monads]
    Let $(\mathsf{C}, \otimes, I, [-,-])$ be a closed monoidal category (for the relevant definitions and notation, see \cite[p. 13, 1.5]{kelly1982basic} (( note : this is also in MacLane ! )); readers unfamiliar with closed monoidal categories may also just assume that $\mathsf{C}=\sets$, $\otimes = \times$, $I=1$ and $[X,Y]=Y^X$). Then we have that
    (( ... ))
\end{example}











\section{Graveyard}

\subsection{Characterisation of $M$-modules}

\begin{lem}[Internal characterisation of locally convex linear $k$-spaces]
    Let $V$ be a linear $k$-space. Then $V$ is locally convex if, and only of, the following two conditions hold:
    \begin{enumerate}[1.]
        \item $\mathscr{l}_0V$ is Hausdorff, meaning that for every non-zero $v\in V$, there is a convex neighbourhood $C$ of $v$ in $V$ such that $0\not\in C$.
        \item $k\mathscr{l}_0V = V$, which means: a subset $U\subseteq V$ is open already if for every compact set $K\subseteq \mathscr{l}_0V$, there exists a convex open set $C\subseteq V$ such that $C\cap K \subseteq U \cap K$.
    \end{enumerate}
\end{lem}
\begin{proof}
    ...
\end{proof}

\begin{prop}
    Every $M$-module is locally convex when considered as a linear $k$-space.
\end{prop}
\begin{proof}
    ...
\end{proof}

\subsection{Locally convex linear $k$-spaces}

Given a locally convex topological vector space (abbreviated LCTVS in the following) $E$, we obtain a linear $k$-space $kE$ by $k$-ification, as continuity of $+:E\times_{\topsp}E\to E$ clearly implies continuity of $+:k(E\times_{\topsp} E) = kE\times kE \to kE$. This leads to the following definition:

\begin{defn}[Locally convex linear $k$-space]
    \text{}
    \begin{enumerate}[1.]
        \item A \emph{locally convex linear $k$-space} is a linear $k$-space $V$ that is the $k$-ification of some locally convex topological vector space $E$, i.e. there exists some LCTVS $E$ such that $V=kE$.
        \item Denote the category of LCTVS with continuous linear maps as morphisms by $\lctvs$ and write $k\lctvs$ for the full subcategory of $\vect$ spanned by locally convex linear $k$-spaces (i.e. $k$-ifications of LCTVS).
        \item Given a locally convex linear $k$-space $V$, let $\unkify(V)$ be the LCTVS whose underlying vector space is that of $V$ and whose topology is generated by the convex open subsets of $V$. (That $\unkify(V)$ is indeed a LCTVS we will show in lemma \ref{unkification_lemma}.) 
        \item Similarly, given a continuous linear map $f:V\to W$ between locally convex linear $k$-spaces, let 
            $$ \unkify(f): \unkify(V) \to \unkify(W) $$
        be the same map as $f$, now considered as a morphism of $LCTVS$. (That $\unkify(f)$ is indeed continuous and hence a morphism of LCTVS, we will also show in lemma \ref{unkification_lemma}.)
        \item This way, we obtain a functor (``un-$k$-ification'')
            $$ \unkify: kLCTVS \to LCTVS. $$
    \end{enumerate}
\end{defn}

The obvious question is now whether un-$k$-ification is indeed a right inverse to the $k$-ification functor
    $$ k: LCTVS \to kLCTVS, $$
as suggested by the name (i.e. whether $k\unkify(V) = V$ for any locally convex linear $k$-space $V$). This will be answered positively in lemma \ref{unkification_left_inverse}. But before we come to that, let us verify the claims made in the above definition.

\begin{lem}\label{unkification_lemma}
    ...
\end{lem}

\begin{lem}\label{unkification_left_inverse}
    ...
\end{lem}

\begin{lem}[$k$-ified Hahn-Banach extension theorem]
    ...
\end{lem}

\begin{lem}[Closed subspaces inherit local convexity.]
    (PROBABLY FALSE) Let $V=kE$ be a locally convex linear $k$-space (with $E$ some LCTVS) and let $W\subseteq V$ be a closed linear subspace. Then $W$ is a locally convex linear $k$-space, as well.
\end{lem}
\begin{proof}
    (DOES NOT WORK) First of all, $W$ is a linear $k$-space, being a closed subspace of $V$. Now, let $\tilde{W}$ be $W$, re-topologised as a subspace of $\unkify(V)$ (which is equal to $E$ by lemma \ref{unkification_left_inverse}). Consider the inclusion
        $$ \iota: \tilde{W} \to \unkify(V)=E$$
    and $k$-ifiy it to obtain
        $$ k\iota: k\tilde{W} \to kE=V.$$
    As subsets of $V$, $k\tilde{W}=W$. Moreover, since the $k$-ification of a closed embedding is a closed  embedding (( THIS IS FLASE )), $k\iota$ is an embedding and so the topologies of $W$ and $k\tilde{W}$ coincide, as well. As a subspace of a LCTVS, $\tilde{W}$, too, is a LCTVS. Therefore, being the $k$-ification of the LCTVS $\tilde{W}$, $W$ is a locally convex linear $k$-space, which is what we wanted to show.
\end{proof}


\subsection{Hahn-Banach-type extension theorem: old try}

\begin{defn}
    A linear $k$-space $V$ is said to have the \emph{extension property} if, and only if, for any closed linear subspace $W \subseteq V$ and any continuous linear functional $\phi\in W^\wedge$ on $W$, $\phi$ has an extension $\tilde{\phi}\in V^\wedge$ to all of $V$.
\end{defn}

\begin{displaycomment}
    One could also wonder about extending linear maps from not-necessarily closed linear subspaces, but this is a different kind of question, which I may add something about later...
\end{displaycomment}

\begin{lem}\label{oplus_extn_lem}
    If $(V_i)_{i\in I}$ is a family of separated-complete linear $k$-spaces, all of whose members have the extension property. Then 
        $$ V := \bigoplus_{i\in I} V_i$$
    has the extension property, as well. 
\end{lem}
\begin{proof}
    Let $W\subseteq V$ be a linear subspace and let $\phi$ be any continuous linear functional on $W$. Denote by 
        $W_i := \iota^{-1}(V_i) \subseteq W$
    the $i$-th factor of $W$, where $\iota: W\hookrightarrow V$ is the inclusion, and let $\phi_i$ be the restriction of $\phi$ to $W_i$. Since $W_i$ is a linear subspace of $V_i$, and $V_i$ has the extension property, by assumption, $\phi_i$ has a continuous linear extension $\tilde{\phi}_i$ to all of $V_i$. Define
        $$ \tilde{\phi} := \bigoplus_{i\in I} \tilde{\phi}_i.$$
    Then $\tilde{\phi}$ is a continuous linear functional on all of $V$. It remains to verify that the restriction of $\tilde{\phi}$ to $W$ is $\phi$. Its restriction to each $W_i$ is $\phi_i$ and hence,
        $$ \tilde{\phi}|_{W} = \bigoplus_{i\in I} \tilde{\phi}_i|_{W_i} = \bigoplus_{i\in I} \phi_i = \phi,$$
    which completes the proof.
\end{proof}

\begin{displaycomment}
    Not quite satisfied with the last step in the above proof. I should add more detail, maybe some commutative diagrams...
\end{displaycomment}

\begin{lem}\label{MX_extn_lem}
    Let $X$ be a compactum. Then $\mnd X$ has the extension property.
\end{lem}
\begin{proof}
    By theorem \ref{Smith_duality}, $\mnd X$ is a locally convex topological vector space, so the assertion follows from the Hahn-Banach extension theorem.
\end{proof}

Recall that a morphism is a category $\mathsf{C}$ is called a \emph{regular epimorphism} if it is the co-equaliser of some pair of morphisms in $\mathsf{C}$ (see \ref{khaus_morphisms_subsec}). 

\begin{lem}\label{reg_epis_in_sclin}
    Let $V,W$ be separated-complete linear $k$-spaces and let $p:V\to W$ be a continuous linear map. Then the following are equivalent:
    \begin{enumerate}[1.]
        \item $p$ is a regular epimorphism in $\sclin$. 
        \item $p$ is the cokernel in $\sclin$ of its kernel. That is, $p$ is the cokernel of the inclusion map
            $$ \iota: \ker p \hookrightarrow V.$$
    \end{enumerate}
\end{lem}
\begin{proof}
    ``1. $\Rightarrow$ 2.'': That $p$ is a regular epimorphism means that there are morphisms $f,g: Z \to V$ such that $p$ is the co-equaliser of $f$ and $g$. To show that $p$ is the cokernel of $\iota$, let $h:V \to S $ be any morphism that vanishes on $\ker p$. We need to verify that there exists a unique morphism $\overline{h}$ such that the diagram,
    % https://q.uiver.app/?q=WzAsMyxbMCwwLCJWIl0sWzEsMCwiVyJdLFsxLDEsIlMiXSxbMCwxLCJwIl0sWzAsMiwiaCIsMl0sWzIsMSwiXFxvdmVybGluZXtofSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
    \begin{equation}\label{cokernel_diag_reg_epi_lem}
    \begin{tikzcd}
	V & W \\
	& S
	\arrow["p", from=1-1, to=1-2]
	\arrow["h"', from=1-1, to=2-2]
	\arrow["{\overline{h}}"', dashed, from=2-2, to=1-2]
    \end{tikzcd}
    \end{equation}
    commutes.
    Let $z \in Z$. Then, by commutativity of the co-equaliser diagram,
    % https://q.uiver.app/?q=WzAsMyxbMSwwLCJWIl0sWzIsMCwiVyJdLFswLDAsIloiXSxbMCwxLCJwIl0sWzIsMCwiZiIsMCx7Im9mZnNldCI6LTF9XSxbMiwwLCJnIiwyLHsib2Zmc2V0IjoxfV1d
    \[\begin{tikzcd}
	Z & V & W,
	\arrow["p", from=1-2, to=1-3]
	\arrow["f", shift left=1, from=1-1, to=1-2]
	\arrow["g"', shift right=1, from=1-1, to=1-2]
    \end{tikzcd}\]
    we have that $p(f(z)-g(z))=0$, i.e. $f(z)-g(z)\in \ker p$. Hence, 
        $$ h(f(z))-h(g(z)) = h(f(z)-g(z)) = 0, $$
    implying that $h\circ f = h \circ g$, as $z\in Z$ was arbitrary. The universal property of the co-equaliser now yields a unique morphism $\overline{h}: S \to V$ making the diagram (\ref{cokernel_diag_reg_epi_lem}) commute, concluding this direction of the proof. \par
    ``2. $\Rightarrow$ 1.'': If $p$ is the co-kernel of $\iota$, then it is the co-equaliser of $\iota$ and the zero map $Z\to V$ and therefore, a regular epimorphism.
\end{proof}

\begin{lem}\label{simul_extn_lemma}
    (( THIS IS FALSE ! ))
    Let $W_1,W_2$ be closed linear subspaces of some linear $k$-Hausdorff space $V$. Then:
    \begin{enumerate}
        \item The addition map 
        $$+|_{ W_1 \oplus W_2}: W_1 \oplus W_2 \to W_1 + W_2, \;\;\; x \oplus y \mapsto x+y$$ 
        is an open map, and hence, the induced (\emph{a priori} only bijective, continuous linear) map
            $$i: W_1 \oplus W_2/\ker(+|_{ W_1 \oplus W_2}) \to W_1 + W_2 $$
        is an \emph{isomorphism} of linear $k$-spaces.
        \item Let $\phi, \psi$ be continuous functionals on $W_1, W_2$, respectively, that coincide on the intersection $W_1 \cap W_2$. Then there is a (unique) continuous functional $\chi$ on $W_1+W_2$ that is a common extension of both $\phi$ and $\psi$ to $W_1+W_2$.
    \end{enumerate}
\end{lem}
\begin{proof} \text{}
    \begin{enumerate}
        \item The unrestricted addition map 
            $$+: V \oplus V \to V, \;\;\; x \oplus y \mapsto x+y $$ 
        is an open map, since it is a split epimorphism (with section $x \mapsto 0 \oplus x$), split epimorphisms are quotient maps (proposition \ref{}) and linear quotient maps are open (proposition \ref{}). Moreover, if we denote by $\iota_1, \iota_2$ the inclusion maps of $W_1,W_2$ into $V$, respectively, then 
            $$ +|_{ W_1 \oplus W_2} = + \circ (\iota_1 \oplus \iota_2) = + \circ (\iota_1 \times \iota_2). $$
        The product of closed embeddings is again a closed embedding (see proposition \ref{khaus_morphisms}) and hence, in particular, it is open onto its image. The claim now follows from the openness of $+$, noted before.
        \item Since $\phi$ and $\psi$ coincide on $W_1 \cap W_2$, the functional $\phi\oplus \psi$ on $W_1 \oplus W_2$ induces a functional $\chi_0$ on $W_1 \oplus W_2/\ker(+|_{ W_1 \oplus W_2})$. Now, $\chi := \chi_0 \circ i^{-1}$ (where $i$ is the isomorphism from the previous point) is the desired simultaneous extension of $\phi$ and $\psi$. 
    \end{enumerate}
\end{proof}

\begin{lem}\label{key_lem_extn}
    If $V,W$ are separated-complete linear $k$-spaces, $p: V\to W$ is a regular epimorphism (in $\sclin$) and $V$ has the extension property, then $W$ has the extension property, as well. 
\end{lem}
\begin{proof}
    We arrange our proof into several steps as follows.
    \begin{enumerate}
        \item $Z\subseteq W$ be any closed linear subspace, and let $\phi$ be any continuous linear functional on $Z$. We would like to show that $\phi$ has an extension $\tilde{\phi}$ to all of $V$.
        \item Note that $p(p^{-1}(Z))\subseteq Z$ and define 
            $$ q: p^{-1}(Z) \to Z, \;\;\; v \mapsto p(v) $$
        by first restricting $p$ to $p^{-1}(Z)$ and then co-restricting the resulting morphism to $Z$. Note that $p^{-1}(Z)$ is a separated-complete linear $k$-space and that $q$ is a continuous linear map.
        \item We can depict our situation as follows:
        % https://q.uiver.app/?q=WzAsNixbMSwwLCJWIl0sWzIsMCwiVyJdLFsxLDEsInBeey0xfShaKSJdLFsyLDEsIloiXSxbMSwyLCJcXG1hdGhiYntLfSJdLFswLDAsIlxca2VyIHAiXSxbMCwxLCJwIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoiZXBpIn19fV0sWzIsMCwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJib3R0b20ifX19XSxbMiwzLCJxIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoiZXBpIn19fV0sWzMsMSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJib3R0b20ifX19XSxbMyw0LCJcXHBoaSIsMCx7ImN1cnZlIjotMX1dLFs1LDAsIiIsMix7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoiYm90dG9tIn19fV0sWzEsNCwiXFxleGlzdHNcXG1hdGhiZns/fSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjozMCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV1d
        \[\begin{tikzcd}
	       {\ker p} & V & W \\
	       & {p^{-1}(Z)} & Z \\
	       & {\mathbb{K}}
	       \arrow["p", two heads, from=1-2, to=1-3]
	       \arrow[hook', from=2-2, to=1-2]
	       \arrow["q"', two heads, from=2-2, to=2-3]
	       \arrow[hook', from=2-3, to=1-3]
	       \arrow["\phi", curve={height=-6pt}, from=2-3, to=3-2]
	       \arrow[hook', from=1-1, to=1-2]
	       \arrow["{\exists\mathbf{?}}"{description, pos=0.3}, dotted, from=1-3, to=3-2]
        \end{tikzcd}\]
        \item Consider the two continuous linear functionals
            $$ \phi \circ q : p^{-1}(Z) \to \mathbb{K}$$
        and the zero functional 
            $$ 0_{\ker p} : \ker p \to \mathbb{K}, \;\;\; x \mapsto 0.$$
        \item $\phi \circ q$ and $0_{\ker p}$ are defined on closed linear subspaces of the linear $k$-space $V$ and agree on their intersection: if $x\in p^{-1}(Z)\cap \ker p$, then 
            $$ \phi\circ q(x) = \phi(p(x)) = \phi(0) = 0 = 0_{\ker p}(x).$$
        \item Hence, according to lemma \ref{simul_extn_lemma}, there is a simultaneous continuous linear extension $\chi$ of both $\phi \circ q$ and $0_{\ker p}$ to the subspace $p^{-1}(Z)+\ker p$ of $V$. We can illustrate all of this in a commutative diagram as follows:
        % https://q.uiver.app/?q=WzAsNyxbMSwwLCJWIl0sWzIsMCwiVyJdLFsxLDEsInBeey0xfShaKSJdLFsyLDEsIloiXSxbMCwwLCJcXGtlciBwIl0sWzAsMSwiXFxrZXIgcCArIHBeey0xfShaKSJdLFsxLDIsIlxcbWF0aGJie0t9Il0sWzAsMSwicCIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFsyLDAsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoiYm90dG9tIn19fV0sWzIsMywicSIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFszLDEsIiIsMix7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoiYm90dG9tIn19fV0sWzQsMCwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJib3R0b20ifX19XSxbMiw1LCIiLDAseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6ImJvdHRvbSJ9fX1dLFs0LDUsIiIsMSx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoiYm90dG9tIn19fV0sWzUsMCwiIiwxLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJib3R0b20ifX19XSxbMyw2LCJcXHBoaSIsMCx7ImN1cnZlIjotMX1dLFsyLDYsIlxccGhpXFxjaXJjIHEiLDJdLFs1LDYsIlxcY2hpIiwyLHsiY3VydmUiOjF9XV0=
        \[\begin{tikzcd}
	       {\ker p} & V & W \\
	       {\ker p + p^{-1}(Z)} & {p^{-1}(Z)} & Z \\
	       & {\mathbb{K}}
	       \arrow["p", two heads, from=1-2, to=1-3]
	       \arrow[hook', from=2-2, to=1-2]
	       \arrow["q"', two heads, from=2-2, to=2-3]
	       \arrow[hook', from=2-3, to=1-3]
	       \arrow[hook', from=1-1, to=1-2]
	       \arrow[hook', from=2-2, to=2-1]
	       \arrow[hook', from=1-1, to=2-1]
	       \arrow[hook', from=2-1, to=1-2]
	       \arrow["\phi", curve={height=-6pt}, from=2-3, to=3-2]
	       \arrow["{\phi\circ q}"', from=2-2, to=3-2]
	       \arrow["\chi"', curve={height=6pt}, from=2-1, to=3-2]
        \end{tikzcd}\]
        \item As $V$ has the extension property, we can further extend $\chi$ to a continuous linear functional $\tilde{\chi}$ on all of $V$ to obtain the commutative diagram,
        % https://q.uiver.app/?q=WzAsNSxbMSwwLCJWIl0sWzIsMCwiVyJdLFsyLDEsIloiXSxbMCwxLCJcXGtlciBwICsgcF57LTF9KFopIl0sWzEsMiwiXFxtYXRoYmJ7S30iXSxbMCwxLCJwIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoiZXBpIn19fV0sWzIsMSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJib3R0b20ifX19XSxbMywwLCIiLDEseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6ImJvdHRvbSJ9fX1dLFsyLDQsIlxccGhpIiwwLHsiY3VydmUiOi0xfV0sWzMsNCwiXFxjaGkiLDIseyJjdXJ2ZSI6MX1dLFswLDQsIlxcdGlsZGV7XFxjaGl9IiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
        \[\begin{tikzcd}
	       & V & W \\
	       {\ker p + p^{-1}(Z)} && Z \\
	       & {\mathbb{K}}
	       \arrow["p", two heads, from=1-2, to=1-3]
	       \arrow[hook', from=2-3, to=1-3]
	       \arrow[hook', from=2-1, to=1-2]
	       \arrow["\phi", curve={height=-6pt}, from=2-3, to=3-2]
	       \arrow["\chi"', curve={height=6pt}, from=2-1, to=3-2]
	       \arrow["{\tilde{\chi}}"', dashed, from=1-2, to=3-2]
        \end{tikzcd}\]
        \item If $x\in \ker p$, then $\tilde{\chi}(x)=\chi(x)=0$, and therefore, since $p$ is the cokernel of its kernel (by lemma \ref{reg_epis_in_sclin}), we can apply the universal property of the cokernel to obtain a morphism $\tilde{\phi}:W\to \mathbb{K}$ such that the following diagram commutes:
        % https://q.uiver.app/?q=WzAsNSxbMSwwLCJWIl0sWzIsMCwiVyJdLFsyLDEsIloiXSxbMCwxLCJcXGtlciBwICsgcF57LTF9KFopIl0sWzEsMiwiXFxtYXRoYmJ7S30iXSxbMCwxLCJwIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoiZXBpIn19fV0sWzIsMSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJib3R0b20ifX19XSxbMywwLCIiLDEseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6ImJvdHRvbSJ9fX1dLFsyLDQsIlxccGhpIiwwLHsiY3VydmUiOi0xfV0sWzMsNCwiXFxjaGkiLDIseyJjdXJ2ZSI6MX1dLFswLDQsIlxcdGlsZGV7XFxjaGl9IiwyXSxbMSw0LCJcXHRpbGRle1xccGhpfSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
        \[\begin{tikzcd}
	       & V & W \\
	       {\ker p + p^{-1}(Z)} && Z \\
	       & {\mathbb{K}}
	       \arrow["p", two heads, from=1-2, to=1-3]
	       \arrow[hook', from=2-3, to=1-3]
	       \arrow[hook', from=2-1, to=1-2]
	       \arrow["\phi", curve={height=-6pt}, from=2-3, to=3-2]
	       \arrow["\chi"', curve={height=6pt}, from=2-1, to=3-2]
	       \arrow["{\tilde{\chi}}"', from=1-2, to=3-2]
	       \arrow["{\tilde{\phi}}", dashed, from=1-3, to=3-2]
        \end{tikzcd}\]
        $\tilde{\phi}$ is the desired extension, by commutativity of the diagram, concluding the proof.
        \end{enumerate}
\end{proof}

\begin{lem}\label{MX_arbit_extn_lem}
    Let $X$ be a $k$-space. Then $MX$ has the extension property.
\end{lem}
\begin{proof}
    Since $X$ is a $k$-space, by lemma \ref{char_k_sp}, there is a family of compacta $(K_i)_{i\in I}$ and a quotient map 
        $$ p: \bigsqcup_{i\in I} K_i \to X. $$
    Quotient maps are equivalently regular epimorphisms (i.e.~the co-equaliser of some pair of morphisms) in $\spaces$ (see proposition \ref{khaus_morphisms} (( WAIT: NOT QUITE THE RIGHT STATEMENT )) ). Since 
        $$ \mnd: \spaces \to \sclin $$
    is a left adjoint (proposition \ref{MX_free_sep_compl_lin_space}), it preserves colimits, and hence, in particular, coproducts and regular epimorphisms. Therefore, 
        $$ \mnd p: \mnd\Big( \bigsqcup_{i\in I} K_i\Big) \to \mnd X $$
    is a regular epimorphism and we have an isomorphism 
        $$ i: \bigoplus_{i\in I} \mnd X_i \cong \mnd\Big( \bigsqcup_{i\in I} X_i\Big).$$
    By lemmas \ref{MX_extn_lem} and \ref{oplus_extn_lem},
        $$ \bigoplus_{i\in I} \mnd X_i $$
    has the extension property. Therefore, $p$ is a regular epimorphism to $MX$ from a separated-complete linear $k$-space having the extension property. Applying lemma \ref{key_lem_extn} then concludes the proof.
\end{proof}

\begin{thm}[Extension Theorem]
    Every separated-complete linear $k$-space has the extension property.
\end{thm}
\begin{proof}
    For any separated-complete linear $k$-space $V$, the integration map
        $$ \smallint{}^V: MV \to V $$
    is a regular epimorphism in $\sclin$ (even a \emph{split} epimorphism with right inverse $\delta_\bullet$). But we have just seen in lemma \ref{MX_arbit_extn_lem} that $MV$ has the extension property, so we can apply lemma \ref{key_lem_extn} again to conclude that $V$ must have the extension property, as well.
\end{proof}

\subsection{Hahn-Banach-type extension theorem: new try}

(DOES NOT WORK EITHER)


\begin{defn}
    Let $V$ be a linear $k$-space. We say that $V$ has the \emph{extension property} if, and only if, for any closed linear subspace $W \subseteq V$ and any continuous linear functional $\phi\in W^\wedge$ on $W$, $\phi$ has an extension $\tilde{\phi}\in V^\wedge$ to all of $V$.
\end{defn}

\begin{displaycomment}
    One could also wonder about extending linear maps from not-necessarily closed linear subspaces, but this is a different kind of question, which I may add something about later...
\end{displaycomment}

The goal is now to show that \emph{every} separated-complete linear $k$-space has the extension property (theorem \ref{extn_thm}). A first observation in this direction is the following lemma.

\begin{lem}\label{extn_emb_lemma}
    For every separated-complete linear $k$-space $V$, there is a family $(X_i)_{i\in I}$ of compacta and a linear closed embedding
        $$ \iota: V \hookrightarrow \prod_{i\in I} C(X_i). $$
    In particular, every separated-complete linear $k$-space admits an embedding into a product (in $\vect$) of Banach spaces. 
\end{lem}
\begin{proof}
    $V$ is separated-complete, so we have a linear closed embedding 
        $$ i: V \hookrightarrow C(V^\wedge). $$
    Since $V^\wedge$ is a $k$-space, by proposition \ref{char_k_sp}, there is a family of compacta $(X_i)_{i\in I}$ and a quotient map 
        $$ p: \bigsqcup_{i\in I} X_i \to V^\wedge. $$
    As an internal hom functor, 
        $C(-)=\mathbb{K}^{(-)}:\khaus^\op \to \khaus $ 
    sends colimits to limits and so it sends regular epimorphisms in $\khaus$ (which are equivalently quotient maps, by proposition \ref{khaus_morphisms}) to regular monomorphisms in $\khaus$ (which are equivalently closed embeddings, again, by proposition \ref{khaus_morphisms}). Similarly, it sends coproducts to products. Hence, applying $C(-)$ to $p$, we obtain a closed embedding 
        $$ j: C(V^\wedge) \hookrightarrow \prod_{i\in I} C(X_i), \;\;\; f \mapsto (X_i \ni x \mapsto f(p(x)))_{i\in I},$$
    which is also linear. The composition 
        $\iota := j \circ i $
    yields the desired closed linear embedding. 
\end{proof}

The extension property is evidently inherited by closed subspaces, so lemma \ref{extn_emb_lemma} reduces our goal to showing that a) any product of linear $k$-spaces with the extension property has the extension property, and b) that each $C(X)$ (with $X$ a compactum) has the extension property. While b) follows from the Hahn-Banach extension theorem for Banach spaces, a) will require two additional lemmas, starting with a rather technical one.

\begin{lem}\label{functls_on_prod_lemma}
    (THIS DOES NOT WORK.)
    Consider the following setup:
    \begin{enumerate}[a.]
        \item Let $(V_i)_{i\in I}$ be a family of linear $k$-spaces, writing 
            $$ V := \prod_{i\in I} V_i$$
        for their product, and $\pi_i:V\to V_i$ for the canonical projection.
        \item Let $W\subseteq V$ be a closed linear subspace and put $W_i := \pi_i(W_i) \subseteq V_i$. 
        \item For each $i\in I$, let $\iota_i: W_i\to V$ be the inclusion of $W_i$ into $W$, given by 
            $$\iota_i(x)_j := \begin{cases}
                x &\text{  if } i=j,\\
                0 &\text{  else,}
            \end{cases}
            $$
        for every $j\in I$. 
        \item Let $\phi\in W^\wedge$ continuous linear functional and for each $i\in I$ let $\phi_i := \phi\circ \iota_i \in W_i^\wedge$.
    \end{enumerate}
    Then for all but finitely many $i\in I$, $\phi_i = 0$. Hence, we can represent $\phi$ as the \emph{finite} sum 
        $$ \phi = \sum_{i\in I} \phi_i \circ \pi_i|_{W}. $$
\end{lem}
\begin{proof}
    \text{}
    \begin{enumerate}
        \item Suppose to the contrary that there is an infinite  number of indices $(i_n)_{n\in \mathbb{N}}$ such that $\phi_{i_n}\not=0$ for all $n\in \mathbb{N}$. 
        \item Then, for every $n\in \mathbb{N}$, there is some $x_n\in W_{i_n}$ such that $\phi_{i_n} \not= 0$.
        \item For every $n\in \mathbb{N}$, put
            $$ y_n := \frac{1}{\phi_{i_n}(x_n)} \iota_{i_n}(x_n) \in W, $$
            $$ s_n := \sum_{k=0}^n y_k \in W. $$
        \item The sequence $(s_n)_{n\in \mathbb{N}}$ converges in $W$. \emph{Proof:}
        \begin{enumerate}
            \item Since $W\subseteq V$ is closed, it suffices to show that $(s_n)_{n\in \mathbb{N}}$ converges in $V$, and this is the case if (and only if) it converges pointwise, i.e.~if for each $j\in I$, $(\pi_j(s_n))_{n\in \mathbb{N}}$ converges in $V_j$. (To see this, use that a convergent sequence in a $k$-space $X$ is equivalently a continuous map $\mathbb{N}\cup \{\infty\} \to X$, where $\mathbb{N}\cup \{\infty\}$ is the one-point compactification, and the universal property of the product.)
            \item For each $j\in I$, $n\in \mathbb{N}$,
                $$ \pi_j(s_n) = \sum_{k=0}^n \frac{1}{\phi_{i_k}(x_k)} \pi_j(\iota_{i_k}(x_k)) = \begin{cases}
                    \;\;\frac{1}{\phi_{i_n}(x_n)}\, x_k &\text{ if } j \in \{i_0, \dots, i_n \}\\
                    \;\;0 &\text{ else.}
                \end{cases}
                $$
            \item Hence, for each $j\in I$, $(\pi_j(s_n))_{n\in \mathbb{N}}$ is eventually constant and hence convergent in $V_i$.
        \end{enumerate}
        \item Using linearity and continuity of $\phi$, we obtain
            $$ \phi\Big( \lim_{n\to \infty} s_n) =  \sum_{n=0}^\infty 
            \phi(y_n) =  \sum_{n=0}^\infty  \frac{1}{\phi_{i_n}(x_n)} \phi(\iota_{i_n}(x_n)) = \sum_{n=0}^\infty 1 = \infty, $$
        the desired contradiction.  
    \end{enumerate}
\end{proof}

\begin{displaycomment}
    Do "sanity checks" on this lemma. E.g. for $W=0$ or $W=V_i$ for some factor, special case of Banach space. Does every functional have to look like this assuming we already knew the duality result? Etc.
\end{displaycomment}

\begin{lem}\label{extn_propty_prod}
    Let $(V_i)_{i\in I}$ be a family of linear $k$-spaces such that each $V_i$ has the extension property. Then the product
        $$ V:=\prod_{i\in I} V_i $$
    has the extension property, as well.
\end{lem}
\begin{proof}
    Let $W\subseteq V$ be a linear $k$-subspace and let $\phi\in W^\wedge$ By lemma \ref{functls_on_prod_lemma}, there is a finite set $J\subseteq I$ of indices such that 
        $$ \phi = \sum_{j\in J} \phi_j \circ \pi_j|_W, $$
    where $\pi_j|_{W}:W\to W_j$ is the (restriction of the) canonical projection and $\phi_j: W_j^\wedge$ is a continuous linear functional on $W_j$. For each $j\in J$, use the extension property of $V_j$ to obtain an extension $\tilde{\phi_j}\in V_j^\wedge$ of $\phi_j\in W_j^\wedge$ to $V_j$. Now, 
        $$ \tilde{\phi} := \sum_{j\in J} \tilde{\phi_j} \circ \pi_j \in V^\wedge $$
    is an extension of $\phi\in W^\wedge$ to all of $V$, since for all $w\in W$,
        $$ \tilde{\phi}(w) = \sum_{j\in J} \tilde{\phi_j}(w) = \sum_{j\in J} \phi_j(w) = \phi(w). $$
\end{proof}

\begin{thm}\label{extn_thm}
    Every separated-complete linear $k$-space has the extension property. 
\end{thm}
\begin{proof}
    Let $V$ be a separated-complete linear $k$-space. According to lemma \ref{extn_emb_lemma}, $V$ admits a closed embedding into a product of Banach spaces. By the Hahn-Banach extension theorem every Banach space has the extension property and by lemma \ref{extn_propty_prod}, a product of linear $k$-spaces having the extension property has the extension property. Hence, $V$ admits embeds as a closed subspace into a linear $k$-space with the extension property. Therefore, $V$ has the extension property, as well. 
\end{proof}



\subsection{Locally convex linear $k$-spaces (new try)}

\begin{defn}[Locally convex linear $k$-space, the functor $\mathscr{l}$]
    \begin{enumerate}[1.]
        \item We call a linear $k$-space $V$ is \emph{locally convex} if, and only if, there is a locally convex topological vector space $E$ such that $V=kE$.
        \item Denote the category of locally convex Hausdorff topological vector spaces with continuous linear maps as morphisms by $\lctvs$ and write $\klctvs$ for the full subcategory of the category $\vect$ of linear $k$-spaces spanned by locally convex linear $k$-spaces.
        \item Note that $k$-ification restricts to a functor
            $$k: \lctvs \to \klctvs, $$
        which we also denote by $k$.
        \item Given a locally convex linear $k$-space $V$ define a locally convex Hausdorff topological vector space $\mathscr{l}V$ as follows. The underlying vector space of $\mathscr{l}V$ is that of $V$ and a basis for the topology of $\mathscr{l}V$ is given by the convex open subsets of $V$. We will show below in lemma \ref{lfunctor_well_def} that $\mathscr{l}V$ is indeed a locally convex Hausdorff topological vector space with this topology, and that given a continuous linear map $f:V\to W$ between locally convex linear $k$-spaces, $f$ is also continuous when viewed as a map $\mathscr{l}f$ from $\mathscr{l}V$ to $\mathscr{l}W$. 
        \item The image of the resulting functor 
            $\mathscr{l}: \klctvs \to \lctvs, $
        i.e.~the full subcategory of $\lctvs$ spanned by spaces of the form $\mathscr{l}V$ for some locally convex linear $k$-space $V$, we denote by $\lklctvs$.
    \end{enumerate}
\end{defn}

\begin{lem}[Well-definedness of $\mathscr{l}$]\label{lfunctor_well_def}
    Let $V$ be a locally convex linear $k$-space. Then $\mathscr{l}V$ is a locally convex Hausdorff topological vector spaces. Moreover, given a continuous linear map $f:W\to V$ to some further locally convex linear $k$-space, $f$ is continuous when viewed as a map $\mathscr{l}f$ from $\mathscr{l}V$ to $\mathscr{l}W$.
\end{lem}
\begin{proof}
    This is suggested (but not verified in full detail) in \cite{seip1979convenient}, just before theorem 2.2.
\end{proof}

\begin{displaycomment}
    Should verify this in detail -- don't find this extremely obvious. 
\end{displaycomment}

\begin{prop}[\cite{seip1979convenient}, Theorem 2.2]
    The functor
        $$ \mathscr{l}: \klctvs \to \lklctvs$$
    is an equivalence (even isomorphism) of categories whose inverse is given by $k$.
\end{prop}


\subsection{A Hahn-Banach-type theorem for separated-complete linear $k$-spaces (another try yet)}

\begin{lem}[Closed subspaces inherit local convexity.]
    (MAYBE JUST FALSE) Let $V=kE$ be a locally convex linear $k$-space (with $E$ some locally convex Hausdorff topological vector space) and let $W\subseteq V$ be a closed linear subspace. Then $W$ is a locally convex linear $k$-space, as well.
\end{lem}
\begin{proof}
    (( use that $k$-ification of closed embedding of Hausdorff spaces is closed embedding? Use $\mathscr{l}$-functor? ))
\end{proof}

(( alternative lemma : $W\subseteq E$ closed implies that the locally convex linear $k$-space $kW$ is a closed linear subspace of $V=kE$. Use case: $V^{\wedge}\subseteq C(V)$? ))

\begin{lem}
    Let $V$ be a locally convex linear $k$-space and let $W\subseteq V$ be a closed linear subspace. Then $W$ is locally convex, as well, and $\mathscr{l}W\subseteq \mathscr{l}V$ is a subspace, i.e.~it carries the (usual) subspace topology.
\end{lem}
\begin{proof}
    (( TODO : prove or delete )) 
\end{proof}

\begin{lem}
    Every locally convex linear $k$-space has the extension property.
\end{lem}
\begin{proof}
    Let $V$ be a locally convex linear $k$-space and let $W\subseteq V$ be a closed linear subspace. Then the inclusion map 
\end{proof}




